Multi-Narrative Semantic Overlap Task: Evaluation and Benchmark

In this paper, we introduce an important yet relatively unexplored NLP task called Multi-Narrative Semantic Overlap (MNSO), which entails generating a Semantic Overlap of multiple alternate narratives. As no benchmark dataset is readily available for this task, we created one by crawling 2,925 narrative pairs from the web and then, went through the tedious process of manually creating 411 different ground-truth semantic overlaps by engaging human annotators. As a way to evaluate this novel task, we first conducted a systematic study by borrowing the popular ROUGE metric from text-summarization literature and discovered that ROUGE is not suitable for our task. Subsequently, we conducted further human annotations/validations to create 200 document-level and 1,518 sentence-level ground-truth labels which helped us formulate a new precision-recall style evaluation metric, called SEM-F1 (semantic F1). Experimental results show that the proposed SEM-F1 metric yields higher correlation with human judgement as well as higher inter-rater-agreement compared to ROUGE metric.

==> SOFSAT Evaluation ARR/Algorithms/sem_f1_metric.tex <==
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %% Automatic Evaluation
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% SEM-F1 algorithm

% \setlength{\textfloatsep}{0.3\baselineskip plus 0.2\baselineskip minus 0.3\baselineskip}
\setlength{\textfloatsep}{8pt}
\begin{algorithm}[!t]\footnotesize 
\caption{Semantic-F1 Metric}
\label{algo:automatic_evaluation}

\begin{algorithmic}[1]

    \State{\textbf{Given} $S_G, S_R, M_E$ }

    \State{$raw_{pV}, raw_{rV} \gets \textsc{CosineSim}(S_G, S_R, M_E)$}
    \Comment{Sentence-wise precision and recall values}
    
    \State{$pV \gets \textsc{Mean}(raw_{pV})$}
    \State{$rV \gets \textsc{Mean}(raw_{rV})$}
    \State{$f_1 \gets \dfrac{2*pV*rV}{pV+rV}$}
    
    % \State{ $pL, pV \gets\textsc{Threshold}(rS_{S_G}, T)$} \Comment{precision}
    % \State{ $rL, rV \gets\textsc{Threshold}(rS_{S_R}, T)$} \Comment{recall}
    
    \State{\textbf{return} $(f_1, pV, rV)$ }
    
\end{algorithmic}

% \end{algorithm}
% \end{figure}
% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % %% Helper Functions
% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[h!]
% \begin{algorithm}[H]
% \caption{Helper Functions}
% \label{algo:helper_functions}

\hrulefill
\begin{algorithmic}[1]
    \Procedure{CosineSim}{$S_G, S_R, M_E$}
        \State{$l_G \gets${No. of sentences in $S_G$}}
        \State{$l_R \gets${No. of sentences in $S_R$}}
        \State{\textbf{init}: $cosSs \gets zeros[l_G, l_R]$; $i \gets 0$}
    
        \For{each sentence $sG$ in $S_G$}
            \State{$E_{sG} \gets M_E(sG)$;$j \gets 0$} 
            \For{each sentence $sR$ in $S_R$}
                \State{$E_{sR} \gets M_E(sR)$} 
                \State{$cosSs[i, j] \gets Cos(E_{sG}, E_{sR})$}
            \EndFor
        \EndFor
        \State{$\boldsymbol{x}\gets$  Row-wise-max($cosSs$)}
        \State{$\boldsymbol{y}\gets$  Column-wise-max($cosSs$)}
        \State{\textbf{return} $(\boldsymbol{x}, \boldsymbol{y})$}
    \EndProcedure
\end{algorithmic}

% \hrulefill
% \begin{algorithmic}[1]
%     \Procedure{Threshold}{$rawSs, T$}
%         \State{\textbf{initialize} $Labels \gets [ ]; W \gets [ ]$}
        
%         \For{each element $e$ in $rawSs$}
%             \If{$e \geq t_u \% $}
%                 \State $Labels.append(P),W.append(1)$
%             \ElsIf{$t_l \% \leq e \leq t_u \% $}
%                 \State $Labels.append(PP);W.append(0.5)$
%             \Else
%                 \State $Labels.append(A);W.append(0)$
%             \EndIf
        
%         \EndFor
        
%         \State{\textbf{return} $Labels, \textsc{Mean}(W)$}
%     \EndProcedure
%     \end{algorithmic}

\end{algorithm}
% \vspace{0mm}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> SOFSAT Evaluation ARR/Algorithms/threshold.tex <==
%% Threshold algorithm
% \setlength{\textfloatsep}{1\baselineskip plus 0.2\baselineskip minus 0.2\baselineskip}
\begin{algorithm}[!htbp] 
\caption{Threshold Function}
\label{algo:threshold}

\begin{algorithmic}[1]
    \Procedure{Threshold}{$rawSs, T$}
        \State{\textbf{initialize} $Labels \gets [ ]$}
        
        \For{each element $e$ in $rawSs$}
            \If{$e \geq t_u \% $}
                \State $Labels.append(P)$
            \ElsIf{$t_l \% \leq e \leq t_u \% $}
                \State $Labels.append(PP)$
            \Else
                \State $Labels.append(A)$
            \EndIf
        
        \EndFor
        
        \State{\textbf{return} $Labels$}
    \EndProcedure
    \end{algorithmic}

\end{algorithm}

==> SOFSAT Evaluation ARR/Sections/allsides_dataset.tex <==

% \vspace{-2mm}
\section{The Benchmark Dataset}
\label{sec:allsides_dataset}
% \vspace{-3mm}
As mentioned in section~\ref{sec:intro}, there is no existing data-set which we could readily use to evaluate the \textit{MNSO} task\footnote{Multi-document summarization datasets can not be utilized in this scenario as their reference summaries do not follow the semantic overlap constraint.}. 
To address this challenge, we crawled data from \href{https://www.allsides.com}{AllSides.com}.
% AllSides.com\footnote{\url{https://www.allsides.com}}
AllSides is a third-party online news forum which exposes people to news and information from all sides of the political spectrum so that the general people can get an ``unbiased'' view of the world. 
To achieve this, AllSides displays each day’s top news stories from news media widely-known to be affiliated with different sides of the political spectrum including “Left” (e.g., New York Times, NBC News),
%  “Center” (e.g., CNBC, Forbes), 
and “Right” (e.g., Townhall, Fox News) wing media.
AllSides also provides their own \textit{factual} description of the reading material, labeled as “Theme” so that readers can see the so-called ``neutral'' point-of-view. 
Table \ref{tab:allsides_dataset} gives an overview of the dataset created by crawling from AllSides.com, which consists of news articles (from at least one “Left” and one “Right” wing media) covering $2,925$ %controversial 
events in total and also having a minimum length of ``theme-description'' to be 15 words. 
Given two narratives (“Left” and “Right”), we used the theme-description as a proxy for ground-truth \textit{TextOverlap}. 
We divided this dataset into testing data (described next) and training data (remaining samples) and their statistics in provided in appendix (table \ref{tab:dataset_statistics}).

\input{Tables/allsides_dataset_overview}

\noindent{\bf Human Annotations\footnote{The dataset and manual annotations can be found in supplementary folder.}:} We decided to involve human volunteers to annotate our testing samples in order to create multiple human-written ground-truth semantic overlaps for each event narrative pairs. This helped in creating a comprehensive testing benchmark for more rigorous evaluation. 
Specifically, we randomly sampled $150$ narrative pairs (one from “Left” wing and one from “Right” wing) and then asked $3$ (three) humans to write a a natural language description which conveys the semantic overlap of the information present in both narratives describing each event. 


After the first round of annotation, we immediately observed a discrepancy among the three annotators in terms of the \textit{real} definition of  ``semantic overlap''. For example, one annotator argued that \textit{Semantic Overlap} of two narratives is non-empty as long as there is an overlap along one of the \textit{5W1H} facets (Who,  What, When, Where, Why and How), while another annotator argued that overlap in only one facet is not enough to decide whether there is indeed a semantic overlap. As an example, one of the annotators wrote only ``Donald Trump'' as the \textit{Semantic Overlap} for a couple of cases where the narratives were substantially different, while others had those cases marked as ``empty set''. 

To mitigate this issue, we only retained the narrative-pairs where at least two of the annotators wrote minimum 15 words as their ground-truth semantic overlap, with the hope that a human written description will contain 15 words or more only in cases where there is indeed a ``significant'' overlap between the two original narratives. 
This filtering step gave us a test set with $137$ samples where each sample had 4 ground-truth semantic overlaps, \textit{one} from AllSides and \textit{three} from human annotators. 
% This filtering step gave us $137$ testing-samples at the end where each sample had 4 ground-truth semantic overlaps, \textit{one} from AllSides and \textit{three} from human annotators. 


% Thus, we decided to redo the entire annotation process such that the annotations don't only focus on single entity. we used the annotation summary length as a proxy to ensure that our manual annotation followed the \textit{5W2H} approach. \naman{This line needs to be modified a bit} 

==> SOFSAT Evaluation ARR/Sections/case_study_rouge.tex <==




% \vspace{-3mm}
\section{Evaluating MNSO Task using ROUGE}
\label{sec:case_study_rouge}
% \vspace{-2mm}
As \textit{ROUGE}~\cite{lin2004rouge} is the most popular metric used today for evaluating summarization techniques; we first conducted a case-study with \textit{ROUGE} as the evaluation metric for MNSO task. %Details on the case-study are presented below.



% \vspace{-3mm}
\subsection{Methods Used in the Case-Study}
\label{subsec:models}
% \vspace{-2mm}
We experimented with multiple SoTA pre-trained abstractive summarization
models as a proxy for \textit{Semantic-Overlap} generators. 
These models are: 1) \textbf{\href{https://huggingface.co/WikinewsSum/bart-large-cnn-multi-en-wiki-news}{BART}} \cite{lewis2019bart}, fine tuned on CNN and multi english Wiki news datasets,
% \footnote{\href{https://huggingface.co/WikinewsSum/bart-large-cnn-multi-en-wiki-news}{WikinewsSum/bart-large-cnn-multi-en-wiki-news}}, 
2) \textbf{\href{https://huggingface.co/google/pegasus-cnn_dailymail}{Pegasus}} \cite{zhang2019pegasus}, fine tuned on CNN and Daily mail dataset, and
% \footnote{\href{https://huggingface.co/google/pegasus-cnn_dailymail}{google/pegasus-cnn\_dailymail}}, 
3) \textbf{\href{https://huggingface.co/WikinewsSum/t5-base-multi-en-wiki-news}{T5}} \cite {raffel2019exploring}, fine tuned on multi english Wiki news dataset. 
% \footnote{\href{https://huggingface.co/WikinewsSum/t5-base-multi-en-wiki-news}{WikinewsSum/t5-base-multi-en-wiki-news}}.  
% Note that, this is not a limitation of this work as our primary goal is to create a benchmark data-set for the \textit{MNSI} task and find a suitable metric for evaluating this task. 
As our primary goal is to construct a benchmark data-set for the \textit{MNSO} task and establish an appropriate metric for evaluating this task, experimenting with only 3 abstractive summarization models is not a barrier to our work.
Proposing a custom method fine-tuned for the \textit{Semantic-Overlap} task is an orthogonal goal to this work and we leave it as a future work. 
Also, we'll use the phrases ``summary'' and ``overlap-summary'' interchangeably from here. 
To generate the summary, we concatenate a narrative pair and feed it directly to the model.


%We use these models to first evaluate the existing summarization evaluation metric, ROUGE and then to further evaluate our proposed metric. since our focus is mostly on the evaluation metric





% \textbf{Generating the summary}:
% In order to handle two input documents, we concatenate them and feed the concatenated input directly to the model. The maximum summary length model hyper-parameter was set to 300 based the max words across samples in the training data. The default values were used for all other hyper-parameters for each respective models.

% \textbf{Post-Processing}: 
% After the generation of model summaries, we did very basic post-processing. For example, for the Pegasus model, the new line character '<n>' was simply replace by blank space following the code from \href{https://github.com/huggingface/transformers}{Huggingface repository}. 
% \santu{One questions goona come. Why did you. not multi document summarizer. }


For evaluation, we first evaluated the machine generated overlap summaries for the 137 manually annotated testing samples using the ROUGE metric \citep{lin2004rouge} and followed the procedure mentioned in the paper to compute the ROUGE-$F_1$ scores with multiple reference summaries.
More precisely, since we have 4 reference summaries, we got 4 precision, recall pairs which are used to compute the corresponding $F_1$ scores. 
For each sample, we took the max of these  $4 F_1$ scores and averaged them out across the test dataset. 
The ROUGE scores can be seen in the table \ref{tab:rouge_score} in appendix. 




\input{Tables/rouge_correlation}
% \vspace{-3mm}
\subsection{Results and Findings}
% \vspace{-2mm}
We computed Pearson's correlation coefficients between each pair of ROUGE-$F_1$ scores obtained using all of the $4$ reference overlap-summaries ($3$ human written summary and $1$ AllSides theme description) to test the robustness of \textit{ROUGE} metric for evaluating the \textit{MNSO} task. 
The corresponding correlations are shown in table \ref{tab:inter_annotator_agreement_rouge}. 
For each annotator pair, we report the maximum (across 3 models) correlation value.
The average correlation value across annotators is $0.36$, $0.33$ and $0.38$ for R1, R2 and RL respectively;
suggesting that ROUGE metric is not stable across multiple human-written overlap-summaries and thus, \textit{unreliable}. 
Indeed, only one out the $6$ different annotator pairs has a value greater than $0.50$ for all the $3$ ROUGE metrics (R1, R2, RL), which is \textit{problematic}.


% %%%%%%%%%%%
% % Rouge Scores
% \begin{table}[!htb]\scriptsize
% \centering
% \vspace{-2mm}
% % \begin{adjustbox}{width=\linewidth,center}
% \begin{tabular}{cccc}
% \toprule
% \textbf{Model} & \textbf{R1} & \textbf{R2} & \textbf{RL} \\
% \midrule
% % BART & 31.7/72.3/40.73 & 20.23/50.35/25.97 
% % & 22.95/57.24/29.95 \\
% % T5 & 28.1/75.97/38.50 & 17.75/55.52/24.63 & 19.93/59.48/27.73 \\
% % Pegasus & 46.13/54.29/46.36 & 28.59/37.47/29.12 & 35.14/48.76/37.41 \\
% BART & 40.73 & 25.97 
% & 29.95 \\
% T5 & 38.50 & 24.63 & 27.73 \\
% Pegasus & 46.36 & 29.12 & 37.41 \\
% \bottomrule
% \end{tabular}
% % \end{adjustbox}
% \vspace{-2mm}
% \caption{Average Rouge-F1 Scores for all the test models across test dataset. For a particular sample, we take the maximum value out of the $4$ F1 scores corresponding to the 4 reference summaries. }
% \vspace{-2mm}
% \label{tab:rouge_score}
% \vspace{-3mm}
% \end{table}




% (percentage p-values confirmed statistical significance) \naman{I took away the p-value}.


%\santu{Frankly, I am not so sure. Without a baseline, we can't say the value is low. Also, if one were to think about it, this is expected since human annotated summaries are quite different from each other. To make a fair comparison, we should concatenate for precision and compute recall individually like what we did for SEM-F1}
%%%%%%%%%%%
% Inter-annotator agreement among rouge-scores



==> SOFSAT Evaluation ARR/Sections/conclusions.tex <==

% \vspace{-3mm}
\section{Conclusions}
\label{conclusions}
% \vspace{-2mm}
In this work, we proposed a new NLP task, called Multi-Narrative Semantic Overlap (\textit{MNSO}) and created a benchmark dataset through meticulous human effort to initiate a new research direction.
As a starting point, we framed the problem as a constrained summarization task and showed that \textit{ROUGE} is not a reliable evaluation metric for this task. 
We further proposed a more accurate metric, called \textit{SEM-F1}, for evaluating \textit{MNSO} task.
Experiments show that SEM-F1 is more robust and yield higher agreement with human judgement.
% , and most importantly, can be computed automatically making it suitable for large-scale evaluation. 

==> SOFSAT Evaluation ARR/Sections/introduction.tex <==

% \vspace{-3mm}
\section{Introduction}
\label{sec:intro}
% \vspace{-2mm}

 %This means that the narration provided by humans contain not only the observed (objective) information about the event, but also their own opinions, making narratives an extremely useful resource for discovering and understanding people's attitudes, perspectives, and preferences. Thus, 

%Human beings can be viewed as subjective sensors who observe real-word events and report relevant information through their own narratives. Thus, multiple alternative narratives provide a robust way to comprehend the complete picture of an event being reported and verify corresponding facts and opinions from different perspectives.  Despite great progress in NLP research in recent years, computers are still far from being able to accurately interpret multiple alternative narratives, which still remains as an open problem. 

In this paper, we look deeper into the challenging yet relatively under-explored area of automated understanding of multiple alternative narratives. 
To be more specific, we formally introduce a new NLP task called \textit{Multi-Narrative Semantic Overlap} (MNSO) and conduct the first systematic study of this task by creating a benchmark dataset as well as proposing a suitable evaluation metric for the task.
% \textit{Multi-Narrative Semantic Intersection} 
MNSO essentially means the task of extracting / paraphrasing / summarizing the \textit{overlapping information} from multiple alternative narratives coming from disparate sources. 
In terms of computational goal, we study the following research question: 

\textit{Given two distinct narratives $N_1$ and $N_2$ of some event $e$ expressed in \textbf{unstructured natural language} format, how can we extract the overlapping information present in both $N_1$ and $N_2$? }




%Given a particular event, multiple narratives of that event often provide different perspective and/or interpretation of the same event. Different narratives usually follow different protagonists often resulting in little variations in tiny details at %finer a granular level. Thus, multiple narratives can help enrich and discover the original story or truth by allowing us to examine the overlap of information, point of views, characters, themes etc. among the multiple narratives. 


%We define this \textit{overlap in information} conveyed by two alternate narratives as the \textit{Semantic Intersection}  for that particular pair of narratives. While, some pair of alternate narratives may have obvious intersections whereas some may not be as clear until the end of the narration.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.85\textwidth]{Images/TextIntersect}
    \vspace{-2mm}
    \caption{A toy use-case for Semantic Overlap Task (\textit{TextOverlap}). 
    A news on topic abortion has been presented by two news media (left-wing and right-wing). 
    ``Green'' Text denotes the overlapping information from both news media, while ``Blue'' and ``Red'' text denotes the respective biases of \textit{left} and \textit{right} wing. 
    A couple of real examples from the benchmark dataset are mentioned in the appendix.}
    \label{fig:semantic_intersection}
    % \vspace{-5mm}
\end{figure*}

% \textcolor{magenta}{
% With the advent of internet, more and more data is being generated on a daily basis. 
% As humans, we convey information through natural language text. 
% Thus, studying this plethora of textual data becomes increasingly important as it can give us important insights into human minds.
% Typically, textual data in an article which consists of a mix of facts and opinions. 
% So when two people describe the same event, their is always going to be differences in their description because of their own biases and thought processes. 
% This poses an interesting questions: Can we come up with a way to extract the common information or facts from two different descriptions of the same event? 
% Can we get some insights about their individual biases and opinions?}
% \santu{This paragraph feels redundant after the first one.}


Figure~\ref{fig:semantic_intersection} shows a toy example of \textit{MNSO} task, where the \textit{TextOverlap}\footnote{We'll be using the terms \textit{TextOverlap} operator and \textit{Semantic Overlap} interchangeably throughout the paper.} ($\cap_{O}$) operation is being applied on two news articles. 
Both articles cover the same story related to the topic ``abortion'', however, they report from different political perspectives, i.e., one from \textit{left} wing and the other from \textit{right} wing. 
For greater visibility, ``Left'' and ``Right'' wing reporting biases are represented by \textit{blue} and \textit{red} text respectively. 
\textit{Green} text denotes the common information in both news articles. 
The goal of \textit{TextOverlap} ($\cap_{O}$) operation is to extract the overlapping information conveyed by the \textit{green} text. 


%These ideas are inspired by the traditional set-theory where various set operations yields the respective information, except that here we are dealing with natural language text. It can be understood from example presented in figure \ref{fig:semantic_intersection} which refers to an interesting use-case of Set-Like \textit{TextIntersect} operator or \textit{Semantic Intersection}. The two news articles are written by two different media outlets reporting on the novel Coronavirus, along with their respective biases as marked by the AllSides.One way to generate a more unbiased summary of the event from these two (politically biased) articles is to identify the overlapping information in both documents, which is nothing but an \textit{Semantic Intersection} \footnote{We'll be using the terms \textit{TextIntersect} operator and \textit{Semantic Intersection} interchangeably throughout the paper.} of the two documents.




At first glance, the MNSO task may appear similar to traditional multi-document summarization task where the goal is to provide an overall summary of the (multiple) input documents; however, the difference is that for \textit{MNSO}, the goal is to provide summarized content with an additional constraint, i.e., the commonality criteria. 
There is no current baseline method as well as existing dataset that exactly match our task; more importantly, it is unclear which one is the right evaluation metric to properly evaluate this task. 
As a starting point, we frame \textit{MNSO} as a constrained  seq-to-seq task where the goal is to generate a natural language output which conveys the overlapping information present in multiple input text documents. 
However, the bigger challenge we need to address first is the following: 1) How can we evaluate this task? and 2) How would one create a benchmark dataset for this task? 
To address these challenges, we make the following contributions in this paper.%\footnote{All the codes will be released upon acceptance.}.



%In this paper, we first present the \textit{Semantic Intersection} problem in detail. The next part focuses on a case-study corresponding to the evaluation of such a system, if there existed one.For the time being, we use multiple state-of-the-art (SoTA) text summarization models as a proxy for \textit{Semantic Intersection}. At the end, we propose a new precision-recall style evaluation evaluation metric, \textbf{SEM-F1}, short for semantic F1. We conduct multiple experiments showing how the new SEM-F1 improves the inter-rated agreement compared to the traditional \textit{ROUGE} metric and also, yields higher correlation among human annotators.

% \vspace{-2mm}
\begin{enumerate}[
leftmargin=*,
% itemsep=0ex,
% partopsep=-1ex,
% parsep=0ex,
]
    \item We formally introduce \textit{Multi-Narrative Semantic Overlap} (MNSO) as a new NLP task and conduct the first systematic study by formulating it as a constrained summarization problem. 
    
    \item We create and release the first benchmark data-set consisting of $2,925$ alternative narrative pairs for facilitating research on the \textit{MNSO} task.  
    Also, we went through the tedious process of manually creating $411$ different ground-truth semantic intersections and conducted further human annotations/validations to create $200$ document-level and $1,518$ sentence-level ground-truth labels to construct the dataset.
    
    \item As a starting point, we experiment with \textit{ROUGE}, a widely popular metric for evaluating text summarization tasks and demonstrate that \textit{ROUGE} is NOT suitable for evaluation of \textit{MNSO} task.
    
    \item We propose a new precision-recall style  evaluation metric, \textbf{SEM-F1} (semantic F1), for evaluating the \textit{MNSO} task. 
    Extensive experiments show that new SEM-F1 improves the inter-rater agreement compared to the traditional \textit{ROUGE} metric, and also, shows higher correlation with human judgments.
    
    % \item Finally, we show how \textbf{SEM-F1} can be used for automated evaluation which can make %facilitate 
    % large scale evaluation practical and feasible. 
\end{enumerate}

==> SOFSAT Evaluation ARR/Sections/motivation.tex <==




\section{Motivation and Applications}
\label{sec:motivation}
% \vspace{-3mm}

Multiple alternative narratives appear frequently across many domains like education, health, military, security and privacy etc (detailed use-cases for each domain are provided in appendix). 
Indeed, MNSO/TextOverlap operation can be very useful to digest such multi-narratives (from various perspectives) at scale and speed and, consequently, enhance the following important tasks as well. 


% Below are some use-cases.

% \noindent \textbf{\underline{Military Intelligence:}} If $A$ and $B$ are two intelligence reports related to a mission from two human agents, the \emph{TextOverlap} operation can help verify the claims in each report w.r.t. the other.

% \noindent \textbf{\underline{Security and Privacy:}} \emph{TextOverlap} operation can enable real-world users to quickly conduct a comparative analysis of multiple privacy policies by mining overlapping clauses from those policies, and thus, help users make informed decisions while choosing from multiple alternative web-services.

% \noindent \textbf{\underline{Medical}:} \textit{TextOverlap} can be applied on clinical notes of patients provided with the same treatment to understand the success/effects of the treatment.

% \noindent \textbf{\underline{Peer-Reviewing}:} Given two peer-review narratives for an article, \textit{TextOverlap} can extract portions of the narratives that agree with each other, which can help prepare a meta-review quickly.

% Here are some of the use-cases of MNSO in various technical areas. 

\noindent \textbf{\underline{Information Retrieval/Search Engines}:} Given a query, one could summarize the common information (\textit{TextOverlap}) from the top $k$ documents fetched by a search engine and display it as additional information to the user. 
%This would immensely help the to quickly parse the information rather than going through each individual article. 
%If they desire, they could further explore the specific articles for more details. 

\noindent \textbf{\underline{Question Answering}:} Given a particular question, the system could aim to provide a more accurate answer based on multiple evidence from various source documents and generate the most common answer by applying \textit{TextOverlap}.

\noindent \textbf{\underline{Robust Translation}:} Suppose you have multiple translation models which translates a given document from language $A$ to language $B$. One could further apply the \textit{TextOverlap} operator on the translated documents and get a robust translation.

In general, MNSO task could be employed in any setting where we have comparative text analysis.

%Thus, the combination of \textbf{\textit{Overlap-Unique-Conflict}} operations can provide a powerful tool for comparative analysis of multi-perspective narratives and help humans digest information from diverse sources quickly. %As human beings, we perceive the real world and report our observations through natural language descriptions aka narratives. In this sense, humans themselves can be regarded as living sensors who observe real-word events and report relevant information through their own narratives. % The unique value of narratives from the perspective of data mining can be explained from the fact that humans are subjective, and far more intelligent than physical sensors. The inevitable subjectivity means that the narration provided by humans contain not only the observed (objective) information about the world, but also their subjective opinions, making narratives an extremely useful resource for discovering and understanding people's attitudes, belief, and preferences. 
% Thus, multiple alternative narratives essentially provide a robust way to comprehend the complete picture of the event being reported and verify corresponding claims and facts from different perspectives.In this regard, \textit{MNSI} can help us figure out the overlapping events and help verifying the facts from multiple different perspectives.



% \noindent{\bf \underline{Problem Formulation}:} What is \textit{Semantic Intersection}? This is indeed a philosophical question and there is no single correct answer. To simplify notations, let us stick to having only two documents $D_A$ and $D_B$ as our input since it can easily be generalized for the case of multiple documents using repeated \textit{TextIntersect} operation. Also, let us define the output as $D_{int} \gets D_A \cap D_B$. Below, we present a set of possible definitions of \textit{Semantic Intersection} to encourage the readers to think more about other alternative definitions. 
% %We first start by looking at the possible definitions of \textit{TextIntersect} and what we are aiming to achieve. 
% %where $D_A$ and $D_B$ are two input documents. 

% All the approaches defined above have their specific use-cases and challenges, however, from a human-centered point of view, they may not reflect how humans generate semantic intersections. A human would mostly express it in the form of natural language and this is why, we frame the \textit{TextIntersect} operator as a constraint summarization problem such that the information of the output summary is present in both the input documents. It can either be extractive summary or abstractive summary or a mixture of both, as per the use case. 

%but lack on common thing which is that this is not how humans would describe the \textit{TextIntersect} operator.

==> SOFSAT Evaluation ARR/Sections/problem_formulation.tex <==
% \vspace{-3mm}
\section{Problem Formulation}
\label{sec:problem_formulation}
% \vspace{-3mm}
What is \textit{Semantic Overlap}? 
This is indeed a philosophical question and there is no single correct answer (various possible definitions are mentioned in appendix section \ref{app_sec:other_definitions}). 
To simplify notations, let us stick to having only two documents $D_A$ and $D_B$ as our input since it can easily be generalized in case of more documents using \textit{TextOverlap} repeatedly. 
Also, let us define the output as $D_{O} \gets D_A \cap_O D_B$. 
A human would mostly express the output in the form of natural language and this is why, we frame the \textit{MNSO} task as a constrained multi-seq-to-seq (text generation) task where the output text only contains information that is present in both the input documents.
We also argue that brevity (minimal repetition) is a desired property of \textit{Semantic Overlap} and thus, we frame \textit{MNSO} task as a constrained summarization problem to ensure brevity.
For example, if a particular piece of information or quote is repeated twice in both the documents, we don't necessarily want it to be present in target overlap summary two times.
The output can either be extractive summary or abstractive summary or a mixture of both, as per the use case. 
This task is inspired by the set-theoretic intersection operator. 
However, unlike set-intersection, our \textit{Text Overlap} does not have to be the \textit{maximal} set. 
The aim is summarize the overlapping information in an abstractive fashion. 
% For example, if a particular piece of information or quote is repeated twice in both the documents, we don't necessarily want it to be present in target overlap summary two times. 
Additionally, \textit{Semantic Overlap} should follow the \textit{commutative} property i.e $D_A \cap_O D_B = D_B \cap_O D_A$.



%We take a human-centric approach to define the \textit{Semantic Intersection}. 

==> SOFSAT Evaluation ARR/Sections/related_works.tex <==


% along with \textit{TextDifference} but the technical details and exact implementation were left as a future work. In our work, we only focus on \textit{TextOverlap}. 
% proposed as part of the framework. 
% However, the technical details and exact implementation were left as a future work. 

% \vspace{-3mm}
\section{Related Works}
\label{sec:related_works}
% \vspace{-3mm}

The idea of semantic text overlap is not entirely new, \citep{karmaker2018sofsat} imagined a hypothetical framework for performing comparative text analysis, where, \textit{TextOverlap} was one of the ``hypothetical'' operators along with \textit{TextDifference}, but the technical details and exact implementation were left as a future work. 
In our work, we only focus on \textit{TextOverlap}.


As \textit{TextOverlap} can be viewed as a multi-document summarization task with additional commonality constraint, text summarization literature is the most relevant to our work.  
Over the years, many paradigms for document summarization have been explored \citep{zhong2019searching}. 
The two most popular among them are \textit{extractive} approaches \citep{cao-etal-2018-retrieve, narayan2018ranking, wu2018learning, zhong2020extractive} and \textit{abstractive} approaches \citep{bae2019summary, hsu2018unified, liu2017generative, nallapati2016abstractive}. 
Some researchers have also tried combining extractive and abstractive approaches \citep{chen2018fast, hsu2018unified, zhang2019pegasus}. 
%Extractive approaches, as the name implies, generate summaries by extracting parts of the original document (usually sentences), while abstractive methods may generate new words or phrases which are not in the original document. 


Recently, encoder-decoder based neural models have become really popular for abstractive summarization \citep{rush2015neural, chopra2016abstractive, zhou2017selective, paulus2017deep}. 
It has become even prevalent to train a general language model on huge corpus of data and then transfer/fine-tune it for the summarization task \citep{radford2019better, devlin-etal-2019-bert, lewis2019bart, xiao2020ernie, yan2020prophetnet, zhang2019pegasus, raffel2019exploring}.
Summary length control for abstractive summarization has also been studied \citep{kikuchi2016controlling, fan2017controllable, liu2018controlling, fevry2018unsupervised, schumann2018unsupervised, makino2019global}. 
In general, multiple document summarization \citep{goldstein2000multi, yasunaga2017graph, zhao2020summpip, ma2020multi, meena2014survey} is more challenging than single document summarization. 
However, \textit{MNSO} task is different from traditional multi-document summarization tasks in that the goal here is to summarize content with an \textit{overlap} constraint, i.e., the output should only contain the common information from both input narratives. 


 

%and are somewhat related to our work since we are also focusing on constrained summarization albeit the constraints are more abstractive and similar to the way a human would think. 
%% Predicate-Argument Alignment

% \vspace{-1mm}
Alternatively, one could aim to recover verb predicate-alignment structure \citep{roth2012aligning, xie2008event, wolfe2013parma} from a sentence and further, use this structure to compute the overlapping information \citep{wang2009recognizing, shibata2012predicate}.
Sentence Fusion is another related area which aims to combine the information from two given sentences with some additional constraints \citep{barzilay1999information, marsi2005explorations, krahmer2008query, thadani2011towards}. 
A related but simpler task is to retrieve parallel sentences \citep{cardon2019parallel, nie1999cross, murdock2005translation} without performing an actual intersection. 
However, these approaches are more targeted towards individual sentences and do not directly translate to arbitrarily long documents. 
Thus, MNSO task is still an open problem and there is no existing dataset, method or evaluation metric that have been systematically studied.


% \vspace{-1mm}
%An idea conceptually similar to our work was applied on visual data \citep{alfassy2019laso}, where the authors developed basic set-operators using neural network based approaches. However, we apply the idea on textual data which comes with entirely different set of challenges. 

% Most recently, it has become even prevalent to train a general language model on huge corpus of data and then transfer/fine-tune it for the summarization task \citep{radford2019better, devlin-etal-2019-bert, lewis2019bart, xiao2020ernie, yan2020prophetnet, zhang2019pegasus, raffel2019exploring}.



% \vspace{-1mm}
Along the evaluation dimension, \textit{ROUGE}~\cite{lin2004rouge} is perhaps the most commonly used metric today for evaluating automated summarization techniques; due to its simplicity and automation. 
However, \textit{ROUGE} has been criticized a lot for primarily relying on lexical overlap~\cite{DBLP:conf/interspeech/Nenkova06,DBLP:conf/naacl/ZhouLMH06,DBLP:conf/lrec/CohanG16} of n-grams. As of today, around $192$ variants of \textit{ROUGE} are available~\cite{DBLP:conf/emnlp/Graham15} including \textit{ROUGE} with word embedding~\cite{DBLP:conf/emnlp/NgA15} and synonym~\cite{DBLP:journals/corr/abs-1803-01937}, graph-based lexical measurement~\cite{DBLP:conf/emnlp/ShafieiBavaniEW18}, Vanilla \textit{ROUGE}~\cite{DBLP:conf/acl/YangLLLL18} and highlight-based \textit{ROUGE}~\cite{DBLP:conf/acl/HardyNV19}. 
However, there has been no study yet whether \textit{ROUGE} metric is appropriate for evaluating the \textit{Semantic Intersection} task, which is one of central goals of our work.

%considers sentence order sensitivity and provides an automatic way of evaluating it as a ranking task, which is the primary goal of our work.

==> SOFSAT Evaluation ARR/Sections/sem_f1.tex <==

% \vspace{-3mm}
\section{Semantic-F1: The New Metric}
\label{subsec:automatic_evaluation}
% \vspace{-3mm}
Human evaluation is costly and time-consuming.
Thus, one needs an automatic evaluation metric for large-scale experiments. 
But, how can we devise an automated metric to perform the sentence-wise precision-recall style evaluation discussed in the previous section? 
To achieve this, we propose a new evaluation metric called \textbf{SEM-F1}. 
The details of our \textbf{SEM-F1} metric are described in algorithm \ref{algo:automatic_evaluation} and the respective notations are mentioned in table \ref{tab:symbol_table}. 
$F_1$ scores are computed by the harmonic mean of the precision ($pV$) and recall ($rV$) values.
Algorithm \ref{algo:automatic_evaluation} assumes only one reference summary but can be trivially extended for multiple references. 
As mentioned previously, in case of multiple references, we concatenate them for precision score computation. 
Recall scores are computed individually for each reference summary and later, an average recall is computed across references. 

The basic intuition behind \textbf{SEM-F1} is to compute the sentence-wise similarity (e.g., cosine similarity using a sentence embedding model) to infer the semantic overlap/intersection between two sentences from both precision and recall perspective and then, combine them into $F_1$ score. 

%The idea of semantic sentence similarity is that the distance between items is based on their meaning or semantic content, and therefore, the cosine similarity between two embedding vectors (i.e. two embedding vectors for two different sentences) can potentially indicate whether these two sentences are semantically similar/close or not. 

\input{Tables/notations}

\input{Algorithms/sem_f1_metric}


% \input{Tables/average_rewards_table}

%%%%%%%%%%%%%
% Reward/Kendall Table
\input{Tables/kendall_reward}
%%%%%%%%%%%%%


% \vspace{-3mm}
\subsection{Is SEM-F1 Reliable?}
% \vspace{-2mm}
\label{subsec:sem_f1_evaluation} 

The SEM-F1 metric computes cosine similarity scores between sentence-pairs from both precision and recall perspectives.
To see whether SEM-F1 metric correlates with human-judgement, we further converted the sentence-wise raw cosine scores into \textit{Presence} (P), \textit{Partial Presence} (PP) and \textit{Absence} (A) labels using some user-defined thresholds as described in algorithm \ref{algo:threshold}. 
This helped us to directly compare the SEM-F1 inferred labels against the human annotated labels.

As mentioned in section \ref{subsec:automatic_evaluation}, we utilized state-of-the-art sentence embedding models to encode sentences from both the model generated summaries and the human written narrative intersections.
To be more specific, we experimented with $3$ sentence embedding models: 
% InferSent-GloVe (\textit{InferSent-V1}) \citep {conneau-EtAl:2017:EMNLP2017},
% InferSent-fastText (\textit{InferSent-V2}) \citep {conneau-EtAl:2017:EMNLP2017}, 
Paraphrase-distilroberta-base-v1 (\textit{P-v1}) \citep{reimers-2019-sentence-bert}, stsb-roberta-large (\textit{STSB}) \citep{reimers-2019-sentence-bert} and universal-sentence-encoder (\textit{USE}) \citep{cer2018universal}.
Along with the various embedding models, we also experimented with multiple threshold values used to predict the sentence-wise \textit{presence (P)}, \textit{partial presence (PP)} and \textit{absence (A)} labels to report the sensitivity of the metric with respect to different thresholds. 
These thresholds are: $(25, 75)$, $(35, 65)$, $(45, 75)$, $(55, 65)$, $(55, 75)$, $(55, 80)$, $(60, 80)$. 
For example, threshold range $(45, 75)$ means that if similarity score $<$ 45\%, infer label "absent", else if similarity score $\geq$ 75\%, infer label "present" and else, infer label ``partial-present''. 
Next, we computed the average precision and recall rewards for 50 samples annotated by label-annotators (L\textsubscript{i}) and the labels inferred by SEM-F1 metric. 
For this, we repeat the procedure of Table~\ref{tab:sentence-wise-annotation-agreeement}, but this time comparing human labels against `SEM-F1 labels'. 
The corresponding results are shown in Table~\ref{tab:average_rewards}.  
% \santu{how about we make that (Inter-Rated-Agreement) a subsection and refer to it.}% Next in Table~\ref{tab:average_rewards}, we repeat the procedure (shown in Table~\ref{tab:sentence-wise-annotation-agreeement}) to calculate the average precision and recall reward scores for the 
% automatically inferred labels by utilizing SEM-F1 for the system generated summaries with respect to each label-annotators. Thus, we can compute the average precision and recall rewards for a given sample and further, for the entire test dataset. 
As we can notice, 
% in table \ref{tab:average_rewards}
the average reward values are consistently high ($\geq 0.50$) for all the $3$ label-annotators (L\textsubscript{i}).  
Moreover, the reward values are consistent/stable across all the $3$ embedding models and threshold values, signifying 
% the robustness of SEM-F1
that SEM-F1 is indeed robust 
across various sentence embeddings and threshold used. %and thus, is  reliable. 

Following the procedure in table \ref{tab:kendall-sentence-wise-annotation-agreeement}, we also  compute the Kendall's Tau between human label annotators and automatically inferred labels using SEM-F1. 
Our results in table \ref{tab:average_rewards} are consistent with reward-based inter-rater-agreement and the correlation values are $\geq 0.50$ with little variation along various thresholds for both precision and recall. 

% \vspace{-3mm}
\input{Tables/sem_f1_scores}
\subsection{SEM-F1 Scores for Random Baselines}
% \vspace{-2mm}
\label{sec: baseline_and_sem_f1_scores}
Here, we present the actual SEM-F1 scores for the three models described in section~\ref{subsec:models} along with scores for two intuitive baselines, namely, 1) Random Overlap 2) Random Annotation. 


\noindent\textbf{Random Overlap:} For a given sample and model, we select a random overlap summary generated by the model out of the other 136 test samples. These random overlaps are then evaluated against 4 reference summaries using SEM-F1. 

\noindent\textbf{Random Annotation:} For a given sample, we select a random reference summary out of the other 4 references among the other 136 test samples. 
The model generated summaries are then compared against these Random Annotations/References to compute SEM-F1 scores as reported in table \ref{tab:sem_f1_scores}.

As we notice, there is approximately 40-45 percent improvement over the baseline scores suggesting SEM-F1 can indeed distinguish \textit{good} from \textit{bad}. 

% \input{Tables/sem_f1_scores}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \vspace{-3mm}
\subsection{Pearson Correlation for SEM-F1}
% \vspace{-2mm}
Following the case-study based on ROUGE in section \ref{sec:case_study_rouge}, we again compute the Pearson's correlation coefficients between each pair of raw SEM-F1 scores obtained using all of the $4$ reference intersection-summaries.
% to test the reliability of \textit{ROUGE} metric for evaluating the \textit{Semantic Intersection} task. 
The corresponding correlations are shown in table \ref{tab:inter_annotator_agreement_sem-f1}. 
For each annotator pair, we report the maximum (across 3 models) correlation value.
The average correlation value across annotators is $0.49$, $0.49$ and $0.54$ for \textbf{P-V1}, \textbf{STSB}, \textbf{USE} embeddings, respectively. 
This shows a clear improvement over the ROUGE metric suggesting that SEM-F1 is more accurate than ROUGE metric.


%%%%%%%%%%%%%
\input{Tables/sem_f1_correlation}
%%%%%%%%%%%


 

==> SOFSAT Evaluation ARR/Sections/story_experiments.tex <==
% \vspace{-3mm}
\section{Can We Do Better than ROUGE?}
% \vspace{-2mm}
\label{sec:summary_label_annotations}
Section \ref{sec:case_study_rouge} shows that ROUGE metric is unstable across multiple reference overlap-summaries. 
Therefore, an immediate question is: Can we come up with a better metric than ROUGE?
% To study this question, we started with manual scoring of machine generated intersections to first establish whether humans agree among themselves or not.  
To investigate this question, we started by manually assessing the machine-generated overlap summaries to check whether humans agree among themselves or not.  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \vspace{-3mm}
\subsection{Different trials of Human Judgement}
% \vspace{-2mm}
\label{subsec:direct_annotation}

\textbf{Assigning a Single Numeric Score:} As an initial trial, we decided to first label 25 testing samples using two human annotators (we call them label annotators $L_1$ and $L_2$). 
Both label-annotators read each of the $25$ narrative pairs as well as the corresponding system generated overlap-summary (generated by fine-tuned BART)
% Both label-annotators also 
and assigned a numeric score between 1-10 (inclusive).
% for all the $25$ system generated intersection-summaries.
%
This number reflects their judgement/confidence about how accurately the system-generated summary captures the \textit{actual} overlap of the two input narratives. 
%
\textit{Note that, the reference overlap summaries were not included in this label annotation process and the label-annotators judged the system-generated summary exclusively with respect to the input narratives}. 
% Worth mentioning, this number reflects their judgement/confidence about how accurately the system-generated summary captures the \textit{actual} intersection of the two input narratives. 
%
To quantify the agreement between human scores, we computed the Kendall rank correlation coefficient (or Kendall's Tau) between two annotator labels since these are ordinal values. 
However, to our disappointment, the correlation value was $0.20$ with p-value being $0.22$\footnote{The higher p-value means that the correlation value is insignificant because of the small number of samples, but the aim is to first find a labelling criterion where human can agree among themselves.}. 
This shows that even human annotators are disagreeing among themselves and we need to come up with a better labelling guideline to reach a reasonable agreement among the human annotators. 
 
On further discussions among annotators, we realized that one annotator only focused on \textit{preciseness} of the intersection summaries, whereas the other annotator took both \textit{precision} and \textit{recall} into consideration. 
Thus, we decided to next assign two  separate scores for precision and recall.


\input{Tables/double_scoring_kendall}
\noindent\textbf{Precision-Recall Inspired Double Scoring:} 
This time, three label-annotators ($L_1$, $L_2$ and $L_3$) assigned two numeric scores between 1-10 (inclusive) for the same set of $25$ system generated summaries. 
These numbers represented their belief about how precise the system-generated summaries were (the precision score) and how much of the actual ground-truth overlap-information was covered by the same (the recall score).
\textit{Also note that, labels were assigned exclusively with respect to the input narratives only}. 
% Again, to establish the agreement among human label annotators, we first computed the F1 scores based on the (normalized) precision-recall (human-provided) scores which were then used to compute the Pearson's correlation coefficients.
As the assigned numbers represent ordinal values (i.e. can't be used to compute $F_1$ score), we compute the Kendall's rank correlation coefficient among the precision scores and recall scores of all the annotator pairs separately. 
% Again, to establish the agreement among human label annotators, we first computed the F1 scores based on the human-provided precision-recall scores which were then used to compute the Kendall's rank correlation coefficients.
% \textit{Also note that, labels were assigned exclusively with respect to the input narratives only}. 
The corresponding correlation values can be seen in the table \ref{tab:two-number-agreeement}. 
As we notice, there is definitely some improvement in agreement among annotators compared to the one number annotation in \ref{subsec:direct_annotation}.
However, the average correlation is still $0.33$ and $0.41$ for precision and recall respectively, much lower than the $0.5$. 

%being the correct precision and recall values for the \textit{intersection} of the input articles. 

%%%%%%%%%%%
% \input{Tables/double_scoring_kendall}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \vspace{-3mm}
\subsection{Sentence-wise Scoring}
\label{subsec:sentence_wise_annotation}
% \vspace{-2mm}
From the previous trials, we realised the downsides of assigning one/two numeric scores to judge an entire system-generated overlap-summary. 
Therefore, as a next step, we decided to assign overlap labels to the each sentence within the system-generated overlap summary and use those labels to compute an overall precision and recall score.

\input{Tables/sentence_wise_scoring_kendall}
\noindent\textbf{Overlap Labels}: Label-annotators ($L_1$, $L_2$ and $L_3$) were asked to look at a machine-generated sentence and determine if the core information conveyed by it is either absent, partially present or present in any of the four reference summaries (provided by ($I_1$, $I_2$, $I_3$ and $I_4$) and respectively, assign the label \textit{A}, \textit{PP} or \textit{P}. 
More precisely, if the human feels there is more than $75\%$ overlap (between each system-generated sentence and reference-summary sentence), assign label \textit{P}, else if the human feels there is less than $25\%$ overlap, assign label \textit{A}, and else, assign \textit{PP} otherwise. 
This sentence-wise labelling was done for 50 different samples (with $506$ sentences in total for system and reference summary), which resulted in total $3\times 506=1,518$ sentence-level ground-truth labels.

To create the overlap labels from precision perspective as described above, we concatenated all the 4 reference summaries to make one big reference summary and asked label-annotators ($L_1$, $L_2$ and $L_3$) to use it as a reference for assigning the overlap labels to each sentence within machine generated summary. 
We argue that if the system could generate a sentence conveying information which is present in any of the references, it should be considered a hit. 
% For recall, we asked label-annotators to assign labels to each sentences in all the 4 reference summaries (provided by ($I_1$, $I_2$, $I_3$ and $I_4$)) with respect to the machine generated summary.
For recall, label-annotators were asked to assign labels to each sentences in each of the 4 reference summaries separately (provided by ($I_1$, $I_2$, $I_3$ and $I_4$)), with respect to the machine generated summary.

% \input{Tables/sentence_wise_scoring_kendall}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent\textbf{Inter-Rater-Agreement}: 
We use the Kendall rank correlation coefficient to compute the agreement among the ordinal labels assigned by human label annotators. 
Since there can be multiple sentences in the system generated or the reference summary, we flatten out the sentence labels and concatenate them for the entire dataset. 
To compute the Kendall Tau, we map the ordinal labels to numerical values using the mapping: $\{P:1, PP:0.5, A:0\}$. 
Table \ref{tab:kendall-sentence-wise-annotation-agreeement} shows that inter-annotator correlation for both precision and recall are $\geq 0.50$ and thus, signifying higher agreement among label annotators. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Tables/reward_function}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent\textbf{Reward-based Inter-Rater-Agreement}: 
Alternatively, 
% It is not possible to compute Pearson's correlation coefficients from the overlap labels (A, P, PP) as they are non-numeric discrete labels. 
% Hence, we again opted to compute inter-annotator agreement in terms of Kendall’s Tau.
% To achieve this, we first define a reward matrix (Table \ref{tab:reward_table}) which is used to compare annotator A's label against annotator B's label for a given machine-generated sentence.
% To achieve this, 
we first define a reward matrix (Table \ref{tab:reward_table}) which is used to compare the label of one annotator (say annotator A) against the label of another annotator (say annotator B) for a given sentence.
This reward matrix acts as a form of correlation between two annotators. 
Once reward has been computed for each sentence, one can compute the average precision and recall rewards for a given sample and accordingly, for the entire test dataset.
The corresponding reward scores can be seen in table \ref{tab:sentence-wise-annotation-agreeement}. 
Both precision and recall reward scores are high ($\geq 0.70$) for all the different annotator pairs, thus signifying, high inter label-annotator agreement. 

We believe, one of the reasons for higher reward/Kendall scores could be that sentence-wise labelling puts less cognitive load on human mind in contrast to the single or double score(s) for the entire overlap summary and accordingly, shows high agreement in terms of human interpretation. 
Similar observation is also noted in \citet{harman-over-2004-effects}. 
% \santu{based on the presentation by Mousumi - ``ask shared meaning between the content in each model summary unit and in the peer summary sentence, and determining how much meaning is shared – a very subjective judgment ==> Need a lot of manual effort.''}



%% Inter-Agreement using Reward Function
%%%%%%%%%%%
\input{Tables/reward_based_agreement}
%%%%%%%%%%%%%%%%%








==> SOFSAT Evaluation ARR/Tables/allsides_dataset_overview.tex <==
%%%%%%%%%%%
% AllSides Dataset Table
% \vspace{-2mm}
\begin{table}[!htb]
\footnotesize
\centering
% \resizebox{\columnwidth}{!}{
\adjustbox{max width=\columnwidth}{%
\begin{tabular}{ll}
% \hline
\toprule
\textbf{Feature} & \textbf{Description} \\
\midrule
% \hline
theme                     & headlines by AllSides \\
theme-description         & news description by AllSides \\
% right/left/center head    & right/left/center news headline \\
% right/left/center-context & right/left/center news description \\ 
right/left head    & right/left news headline \\
right/left context & right/left news description \\
\bottomrule
% \hline
\end{tabular}
}
% \vspace{-2mm}
\caption{Overview of dataset scraped from AllSides}
\label{tab:allsides_dataset}
\vspace{-2mm}
\end{table}

==> SOFSAT Evaluation ARR/Tables/average_rewards_table.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Reward/Kendall Table
\begin{table*}[!t]\footnotesize
\begin{subtable}[h]{\textwidth}
\centering
\ra{1.1}
\adjustbox{max width=\textwidth}{%
\begin{tabular}{p{1.3cm}cccccccc}
%% ------------------------------
%% SIM 3
\toprule
\multicolumn{9}{c}{\textbf{Machine-Human Agreement in terms of Reward Function}}  \\
\cmidrule{3-9}
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{c}{$\mathbf{T=(25, 75)}$} & \multicolumn{1}{c}{$\mathbf{T=(35, 65)}$} & \multicolumn{1}{c}{$\mathbf{T=(45, 75)}$}& \multicolumn{1}{c}{$\mathbf{T=(55, 65)}$} & \multicolumn{1}{c}{$\mathbf{T=(55, 75)}$} & \multicolumn{1}{c}{$\mathbf{T=(55, 80)}$} & \multicolumn{1}{c}{$\mathbf{T=(60, 80)}$}\\ 
\midrule
\multicolumn{9}{c}{\textbf{\textit{Sentence Embedding: P-v1}}}  \\
\midrule

\multirow{3}{*}{\parbox{1.3 cm}{\textbf{Precision Reward}}}
& L\textsubscript{1} &
$\SI{0.73 \pm 0.27}{}$ & $\SI{0.81 \pm 0.25}{}$ & 
$\SI{0.77 \pm 0.26}{}$ & $\SI{0.85 \pm 0.23}{}$ & 
$\SI{0.8 \pm 0.24}{}$ & $\SI{0.77 \pm 0.24}{}$ & 
$\SI{0.77 \pm 0.26}{}$ \\ 
% \cline{ 2- 9}

 & L\textsubscript{2} &
$\SI{0.72 \pm 0.3}{}$ & $\SI{0.73 \pm 0.29}{}$ & 
$\SI{0.73 \pm 0.3}{}$ & $\SI{0.78 \pm 0.27}{}$ & 
$\SI{0.79 \pm 0.27}{}$ & $\SI{0.75 \pm 0.26}{}$ & 
$\SI{0.73 \pm 0.29}{}$ \\ 
% \cline{ 2- 9}

 & L\textsubscript{3} &
$\SI{0.81 \pm 0.23}{}$ & $\SI{0.86 \pm 0.21}{}$ & 
$\SI{0.79 \pm 0.24}{}$ & $\SI{0.78 \pm 0.28}{}$ & 
$\SI{0.74 \pm 0.28}{}$ & $\SI{0.69 \pm 0.28}{}$ & 
$\SI{0.69 \pm 0.27}{}$ \\ 
\midrule
%----------
\multirow{3}{*}{\parbox{1.3 cm}{\textbf{Recall Reward}}} 
& L\textsubscript{1} &
$\SI{0.66 \pm 0.19}{}$ & $\SI{0.79 \pm 0.16}{}$ & 
$\SI{0.75 \pm 0.16}{}$ & $\SI{0.76 \pm 0.18}{}$ & 
$\SI{0.71 \pm 0.17}{}$ & $\SI{0.66 \pm 0.17}{}$ & 
$\SI{0.61 \pm 0.18}{}$ \\ 
% \cline{ 2- 9}

 & L\textsubscript{2} &
$\SI{0.67 \pm 0.19}{}$ & $\SI{0.78 \pm 0.16}{}$ & 
$\SI{0.76 \pm 0.15}{}$ & $\SI{0.73 \pm 0.19}{}$ & 
$\SI{0.72 \pm 0.18}{}$ & $\SI{0.7 \pm 0.18}{}$ & 
$\SI{0.65 \pm 0.21}{}$ \\ 
% \cline{ 2- 9}

 & L\textsubscript{3} &
$\SI{0.66 \pm 0.15}{}$ & $\SI{0.72 \pm 0.17}{}$ & 
$\SI{0.68 \pm 0.17}{}$ & $\SI{0.68 \pm 0.22}{}$ & 
$\SI{0.64 \pm 0.2}{}$ & $\SI{0.59 \pm 0.19}{}$ & 
$\SI{0.57 \pm 0.2}{}$ \\ 

%% ------------------------------
\midrule
%% ------------------------------
%% SIM 4
\multicolumn{9}{c}{\textbf{\textit{Sentence Embedding: STSB}}}  \\
\midrule
\multirow{3}{*}{\parbox{1.3 cm}{\textbf{Precision Reward}}}
& L\textsubscript{1} &
$\SI{0.75 \pm 0.29}{}$ & $\SI{0.75 \pm 0.29}{}$ & 
$\SI{0.75 \pm 0.29}{}$ & $\SI{0.75 \pm 0.29}{}$ & 
$\SI{0.75 \pm 0.29}{}$ & $\SI{0.75 \pm 0.3}{}$ & 
$\SI{0.75 \pm 0.23}{}$ \\ 
% \cline{ 2- 9}

 & L\textsubscript{2} &
$\SI{0.63 \pm 0.32}{}$ & $\SI{0.63 \pm 0.31}{}$ & 
$\SI{0.63 \pm 0.32}{}$ & $\SI{0.63 \pm 0.31}{}$ & 
$\SI{0.63 \pm 0.32}{}$ & $\SI{0.64 \pm 0.32}{}$ & 
$\SI{0.64 \pm 0.32}{}$ \\ 
% \cline{ 2- 9}

 & L\textsubscript{3} &
$\SI{0.81 \pm 0.23}{}$ & $\SI{0.82 \pm 0.23}{}$ & 
$\SI{0.81 \pm 0.23}{}$ & $\SI{0.82 \pm 0.23}{}$ & 
$\SI{0.81 \pm 0.23}{}$ & $\SI{0.81 \pm 0.22}{}$ & 
$\SI{0.81 \pm 0.22}{}$ \\ 
\midrule
%----------
\multirow{3}{*}{\parbox{1.3 cm}{\textbf{Recall Reward}}} 
& L\textsubscript{1} &
$\SI{0.66 \pm 0.21}{}$ & $\SI{0.67 \pm 0.21}{}$ & 
$\SI{0.66 \pm 0.21}{}$ & $\SI{0.68 \pm 0.21}{}$ & 
$\SI{0.67 \pm 0.21}{}$ & $\SI{0.65 \pm 0.21}{}$ & 
$\SI{0.66 \pm 0.21}{}$ \\ 
% \cline{ 2- 9}

 & L\textsubscript{2} &
$\SI{0.57 \pm 0.2}{}$ & $\SI{0.58 \pm 0.21}{}$ & 
$\SI{0.57 \pm 0.2}{}$ & $\SI{0.59 \pm 0.2}{}$ & 
$\SI{0.59 \pm 0.2}{}$ & $\SI{0.58 \pm 0.2}{}$ & 
$\SI{0.58 \pm 0.21}{}$ \\ 
% \cline{ 2- 9}

 & L\textsubscript{3} &
$\SI{0.67 \pm 0.19}{}$ & $\SI{0.67 \pm 0.2}{}$ & 
$\SI{0.67 \pm 0.19}{}$ & $\SI{0.68 \pm 0.2}{}$ & 
$\SI{0.68 \pm 0.19}{}$ & $\SI{0.67 \pm 0.18}{}$ & 
$\SI{0.68 \pm 0.18}{}$ \\ 
%% ------------------------------
\midrule
%% ------------------------------
%% SIM 5
\multicolumn{9}{c}{\textbf{\textit{Sentence Embedding: USE}}}  \\
\midrule

\multirow{3}{*}{\parbox{1.3 cm}{\textbf{Precision Reward}}}
& L\textsubscript{1} &
$\SI{0.76 \pm 0.29}{}$ & $\SI{0.77 \pm 0.3}{}$ & 
$\SI{0.78 \pm 0.27}{}$ & $\SI{0.8 \pm 0.28}{}$ & 
$\SI{0.8 \pm 0.27}{}$ & $\SI{0.77 \pm 0.27}{}$ & 
$\SI{0.8 \pm 0.27}{}$ \\ 
% \cline{ 2- 9}

 & L\textsubscript{2} &
$\SI{0.69 \pm 0.32}{}$ & $\SI{0.66 \pm 0.32}{}$ & 
$\SI{0.71 \pm 0.3}{}$ & $\SI{0.68 \pm 0.3}{}$ & 
$\SI{0.72 \pm 0.3}{}$ & $\SI{0.76 \pm 0.29}{}$ & 
$\SI{0.78 \pm 0.29}{}$ \\ 
% \cline{ 2- 9}

 & L\textsubscript{3} &
$\SI{0.82 \pm 0.24}{}$ & $\SI{0.85 \pm 0.22}{}$ & 
$\SI{0.85 \pm 0.23}{}$ & $\SI{0.86 \pm 0.21}{}$ & 
$\SI{0.85 \pm 0.23}{}$ & $\SI{0.82 \pm 0.23}{}$ & 
$\SI{0.78 \pm 0.25}{}$ \\ 
\midrule
%----------
\multirow{3}{*}{\parbox{1.3 cm}{\textbf{Recall Reward}}} 
& L\textsubscript{1} &
$\SI{0.64 \pm 0.19}{}$ & $\SI{0.67 \pm 0.19}{}$ & 
$\SI{0.68 \pm 0.19}{}$ & $\SI{0.7 \pm 0.21}{}$ & 
$\SI{0.69 \pm 0.22}{}$ & $\SI{0.64 \pm 0.2}{}$ & 
$\SI{0.65 \pm 0.21}{}$ \\ 
% \cline{ 2- 9}

 & L\textsubscript{2} &
$\SI{0.62 \pm 0.19}{}$ & $\SI{0.63 \pm 0.2}{}$ & 
$\SI{0.66 \pm 0.18}{}$ & $\SI{0.66 \pm 0.21}{}$ & 
$\SI{0.68 \pm 0.2}{}$ & $\SI{0.68 \pm 0.19}{}$ & 
$\SI{0.69 \pm 0.21}{}$ \\ 
% \cline{ 2- 9}

 & L\textsubscript{3} &
$\SI{0.64 \pm 0.16}{}$ & $\SI{0.68 \pm 0.19}{}$ & 
$\SI{0.66 \pm 0.16}{}$ & $\SI{0.69 \pm 0.2}{}$ & 
$\SI{0.65 \pm 0.19}{}$ & $\SI{0.6 \pm 0.17}{}$ & 
$\SI{0.6 \pm 0.18}{}$ \\ 
\bottomrule
%% ------------------------------

\end{tabular}
}
\caption{Average Precision and Recall reward/correlation (mean $\pm$ std) between label-annotators (L\textsubscript{i}) and automatically inferred labels using SEM-F1. The results are shown for different embedding models (\ref{subsec:sem_f1_evaluation}) and multiple threshold levels $T=(t_l, t_u)$. For all the annotators L\textsubscript{i} ($i \in \{1, 2, 3\}$), correlation numbers are quite high ($\geq 0.50$).
Moreover, the reward values are consistent/stable across all the $5$ embedding models and threshold values.}
\label{tab:average_rewards_score}
\end{subtable}
% -----------------------
\hfill
\\
\\
% -----------------------
\begin{subtable}[h]{\textwidth}
\centering
\ra{1.1}
\adjustbox{max width=\textwidth}{%
\begin{tabular}{p{1.3cm}cccccccc}


%% ------------------------------
%% SIM 3
\toprule
\multicolumn{9}{c}{\textbf{Machine-Human Agreement in terms of Kendall Rank Correlation}}  \\
\cmidrule{3-9}
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{c}{$\mathbf{T=(25, 75)}$} & \multicolumn{1}{c}{$\mathbf{T=(35, 65)}$} & \multicolumn{1}{c}{$\mathbf{T=(45, 75)}$}& \multicolumn{1}{c}{$\mathbf{T=(55, 65)}$} & \multicolumn{1}{c}{$\mathbf{T=(55, 75)}$} & \multicolumn{1}{c}{$\mathbf{T=(55, 80)}$} & \multicolumn{1}{c}{$\mathbf{T=(60, 80)}$}\\
\midrule
\multicolumn{9}{c}{\textbf{\textit{Sentence Embedding: P-v1}}}  \\
\midrule
\multirow{3}{*}{\parbox{1.3 cm}{\textbf{Precision Reward}}}
& L\textsubscript{1} &
$0.55$ & $0.6$ & $0.58$ & $0.59$ & $0.57$ & $0.56$ & $0.54$ \\ 
% \cline{ 2- 9}

 & L\textsubscript{2} &
$0.61$ & $0.67$ & $0.63$ & $0.67$ & $0.64$ & $0.67$ & $0.68$ \\
% \cline{ 2- 9}

 & L\textsubscript{3} &
 $0.54$ & $0.62$ & $0.56$ & $0.64$ & $0.6$ & $0.56$ & $0.52$ \\
\midrule
%----------
\multirow{3}{*}{\parbox{1.3 cm}{\textbf{Recall Reward}}} 
& L\textsubscript{1} &
$0.53$ & $0.64$ & $0.66$ & $0.62$ & $0.61$ & $0.62$ & $0.59$ \\
% \cline{ 2- 9}

 & L\textsubscript{2} &
$0.55$ & $0.64$ & $0.67$ & $0.63$ & $0.63$ & $0.64$ & $0.61$ \\
% \cline{ 2- 9}

 & L\textsubscript{3} &
$0.54$ & $0.65$ & $0.64$ & $0.66$ & $0.65$ & $0.65$ & $0.61$ \\
%% ------------------------------
\midrule
%% ------------------------------
%% SIM 4
\multicolumn{9}{c}{\textbf{\textit{Sentence Embedding: STSB}}}  \\
\midrule

\multirow{3}{*}{\parbox{1.3 cm}{\textbf{Precision Reward}}}
& L\textsubscript{1} &
$0.57$ & $0.67$ & $0.58$ & $0.66$ & $0.6$ & $0.57$ & $0.58$ \\
% \cline{ 2- 9}

 & L\textsubscript{2} &
$0.66$ & $0.63$ & $0.65$ & $0.63$ & $0.7$ & $0.63$ & $0.6$ \\
% \cline{ 2- 9}

 & L\textsubscript{3} &
$0.56$ & $0.57$ & $0.58$ & $0.56$ & $0.59$ & $0.57$ & $0.56$ \\
\midrule
%----------
\multirow{3}{*}{\parbox{1.3 cm}{\textbf{Recall Reward}}} 
& L\textsubscript{1} &
$0.55$ & $0.65$ & $0.64$ & $0.62$ & $0.62$ & $0.61$ & $0.59$ \\
% \cline{ 2- 9}

 & L\textsubscript{2} &
$0.56$ & $0.65$ & $0.65$ & $0.63$ & $0.63$ & $0.64$ & $0.63$ \\
% \cline{ 2- 9}

 & L\textsubscript{3} &
$0.54$ & $0.59$ & $0.61$ & $0.57$ & $0.58$ & $0.57$ & $0.54$ \\
%% ------------------------------
\midrule
%% ------------------------------
%% SIM 5
\multicolumn{9}{c}{\textbf{\textit{Sentence Embedding: USE}}}  \\
\midrule

\multirow{3}{*}{\parbox{1.3 cm}{\textbf{Precision Reward}}}
& L\textsubscript{1} &
$0.58$ & $0.62$ & $0.6$ & $0.61$ & $0.59$ & $0.62$ & $0.65$ \\
% \cline{ 2- 9}

 & L\textsubscript{2} &
$0.68$ & $0.7$ & $0.68$ & $0.68$ & $0.68$ & $0.7$ & $0.73$ \\
% \cline{ 2- 9}

 & L\textsubscript{3} &
$0.66$ & $0.67$ & $0.65$ & $0.64$ & $0.63$ & $0.53$ & $0.56$ \\
\midrule
%----------
\multirow{3}{*}{\parbox{1.3 cm}{\textbf{Recall Reward}}} 
& L\textsubscript{1} &
$0.53$ & $0.59$ & $0.56$ & $0.61$ & $0.62$ & $0.61$ & $0.6$ \\
% \cline{ 2- 9}

 & L\textsubscript{2} &
$0.54$ & $0.6$ & $0.61$ & $0.62$ & $0.64$ & $0.64$ & $0.62$ \\
% \cline{ 2- 9}

 & L\textsubscript{3} &
$0.52$ & $0.6$ & $0.58$ & $0.61$ & $0.61$ & $0.6$ & $0.6$ \\
\bottomrule
%% ------------------------------

\end{tabular}
}
\caption{Average Precision and Recall Kendall Tau between label-annotators (L\textsubscript{i}) and automatically inferred labels using SEM-F1. The results are shown for different embedding models (\ref{subsec:sem_f1_evaluation}) and multiple threshold levels $T=(t_l, t_u)$. For all the annotators L\textsubscript{i} ($i \in \{1, 2, 3\}$), correlation numbers are quite high ($\geq 0.50$).
Moreover, the reward values are consistent/stable across all the $5$ embedding models and threshold values.
All values are statistically significant at p-value<0.05.  
}
\label{tab:average_kendall_scores}
\end{subtable}
\caption{Machine-Human Agreement}
\label{tab:raw_average_rewards}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> SOFSAT Evaluation ARR/Tables/double_scoring_kendall.tex <==
% Two-number inter-agreement
\begin{table}[!t]\scriptsize %[!htb]
\centering
% \vspace{-1mm}
%\adjustbox{max width=\columnwidth}{%
% \begin{tabular}{cccc} %cccc
% \toprule
% % \multicolumn{4}{c}{\textbf{Kendall's Rank Correlation among label annotators}} \\
% % & \multicolumn{3}{c}{\textbf{Double Score}} && \multicolumn{3}{c}{\textbf{Sentence-wise Score}} \\ 
% % \midrule
% (L\textsubscript{1}, L\textsubscript{2}) & (L\textsubscript{2}, L\textsubscript{3}) & (L\textsubscript{1}, L\textsubscript{3}) & \textbf{Average}\\
% \cmidrule{1-4} %\cmidrule{6-8} 
% 0.30 (0.04) & 0.45 (0.00) & 0.10 (0.51) & $\mathbf{0.28}$ \\
% \bottomrule
% \end{tabular}

\begin{tabular}{cccccc}
\toprule
\multicolumn{6}{c}{\textbf{Human agreement in terms of Kendall Tau}} \\
\cmidrule{2-6}
& \multicolumn{2}{c}{\textbf{Precision}} && \multicolumn{2}{c}{\textbf{Recall}} \\ \midrule
& L\textsubscript{1} & L\textsubscript{2} && L\textsubscript{1} & L\textsubscript{2} \\
\cmidrule{2-3} \cmidrule{5-6} 
%L\textsubscript{1} & --- &  &  && --- & &  \\ 
L\textsubscript{2} & $0.52$ & --- && $0.37$ & ---\\
L\textsubscript{3} & $0.18$ & $0.29$ && $0.31$ & $0.54$\\ 

\cmidrule{1-6}
\textbf{Average} & 
\multicolumn{2}{c}{$\mathbf{0.33}$} &&
\multicolumn{2}{c}{$\mathbf{0.41}$} \\

\bottomrule
\end{tabular}

% \vspace{-1mm}
\caption{Kendall's rank correlation coefficients among the precision and recall scores for pairs of human annotators ($25$ samples). L\textsubscript{i} refers to the $i^{th}$ label annotator.}% Human agreement have definitely improved compared to the one number annotation in \ref{subsec:direct_annotation} but the average correlation value is still $0.43$ which is even less than half. \santu{Fix Align or Join table 4 and 5}}
\label{tab:two-number-agreeement}
\vspace{-4mm}
\end{table}

==> SOFSAT Evaluation ARR/Tables/intersection_examples.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Reward/Kendall Table
\begin{table*}[!htb]\small
% \begin{subtable}[h]{\textwidth}
\centering
%% IMP: Caption has to be at the top. Otherwise, counter is 1 less

\ra{1.2}
\adjustbox{max width=\textwidth}{%
\begin{tabular}{C{0.3cm} | C{3.5cm} | C{3.5cm} | C{3.5cm} | C{5.5cm}} %| m{0.8cm} | m{2cm}}
\toprule
\textbf{Idx} & \multicolumn{2}{c|}{$\mathbf{D_1}$} &
\multicolumn{2}{c}{$\mathbf{D_2}$} \\
\cmidrule{1-5}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Sample 1
\multirow{4}{*}{$\mathbf{1}$} & 
\multicolumn{2}{C{8cm}|}{
% %% -----------------------------------------
%% D1
\hlgreen{
WASHINGTON -- U.S. intelligence and law enforcement agencies have confirmed that President Donald Trump's campaign aides and associates had constant contact with Russian intelligence officials before the election, directly contradicting public statements made by top administration officials. 
}
On Jan. 15, shortly before Trump took office, Vice President Mike Pence repeatedly said on television that there were zero contacts between the campaign and Russian officials. 
$\mathbf{\dotso}$
% "Just to button up one question, did any adviser or anybody in the Trump campaign have any contact with the Russians who were trying to meddle in the election?" 
% CBS "Face the Nation" host John Dickerson asked. 
% "Of course not," Pence replied. 
\hlgreen{
Pence also answered "of course not" when asked a similar question that day by "Fox News Sunday" host Chris Wallace
$\mathbf{\dotso}$
% , adding, "All the contact by the Trump campaign and associates were with the American people." 
Trump himself also denied these interactions
$\mathbf{\dotso}$
% , according to NBC News on Jan. 11: Trump did not specifically address questions regarding whether members of his staff were in contact with Russian officials during the campaign. 
% When NBC News repeated that question to Trump afterwards as the president-elect approached the elevator to exit the room, he answered "No." On Tuesday, White House Press Secretary Sean Spicer seemed to stand by those earlier denials. 
}
"There's nothing that would conclude me that anything different has changed with respect to that time period," Spicer said. 
$\mathbf{\dotso}$
% .@PressSec Sean Spicer tells @jonkarl nobody on the Trump campaign had contact with Russia before the election https://t.co/LBw3Bd5Htk pic.twitter.com/S9H8fgFA2j -- ABC News Politics (@ABCPolitics) February
%% -----------------------------------------
} &
\multicolumn{2}{C{8cm}}{
%% -----------------------------------------
%% D2
\hlgreen{
President Trump said Wednesday that new reports saying his associates had contact with Russian officials during last year's campaign are "non-sense"} and accused the U.S. intelligence community of illegally leaking information to news outlets. 
\hlgreen{
"This Russian connection non-sense} is merely an attempt to cover-up the many mistakes made in Hillary Clinton's losing campaign," Mr. Trump tweeted. 
$\mathbf{\dotso}$
% "Information is being illegally given to the failing @nytimes \& @washingtonpost by the intelligence community (NSA and FBI?).Just like Russia," he also tweeted. 
% He said the "real scandal" is that the intelligence community is giving out classified information "like candy." 
% "The real scandal here is that classified information is illegally given out by 'intelligence' like candy. Very un-American!" the president tweeted. 
% He also said that the "fake news media" is "going crazy" with conspiracy theories and "blind hatred" and declared CNN and MSNBC "unwatchable." "The fake news media is going crazy with their conspiracy theories and blind hatred. @MSNBC \& @CNN are unwatchable. @foxandfriends is great!" Mr. Trump tweeted, referring to Fox News' morning show. 
% The missives comes as multiple news outlets, including CNN and the New York Times, reported Tuesday that Russian officials were in touch with members of Mr. Trump's team during the presidential campaign last year. 
% Advisers close to Mr. Trump were in "constant communication during the campaign with Russians known to US intelligence," CNN reported. 
Among those supposedly communicating with Russian nationals was former Trump campaign chairman Paul Manafort, the report said. 
\hlgreen{Mr. Manafort denied that he ever knowingly talked to any intelligence official "or anyone}
%% -----------------------------------------
} \\
\cmidrule{2-5}
& \multicolumn{4}{c}{\textbf{Overlap}} \\
& \multicolumn{1}{c}{\textbf{A\textsubscript{1}}} &
  \multicolumn{1}{c}{\textbf{A\textsubscript{2}}} &
  \multicolumn{1}{c}{\textbf{A\textsubscript{3}}} &
  \multicolumn{1}{c}{\textbf{AllSides}}
  \\

% \multicolumn{1}{c}{\multirow{2}{*}{$\mathbf{D_1}$}} &
% \multicolumn{1}{c}{\multirow{2}{*}{$\mathbf{D_2}$}} &
% \multicolumn{4}{c}{\textbf{Overlap}} \\
% &&\multicolumn{1}{c}{\textbf{A\textsubscript{1}}} &
%  \multicolumn{1}{c}{\textbf{A\textsubscript{2}}} &
%  \multicolumn{1}{c}{\textbf{A\textsubscript{3}}} &
%  \multicolumn{1}{c}{\textbf{AllSides}}
% \\
\cmidrule{2-5}
&
%% A1
President Trump and the Trump administration deny allegations that advisers close to Trump were in constant communication during the campaign with Russians known to US intelligence.
&
%% A2
Trump denied climas that advisers close to him were in "constant communication during the campaign with Russians known to US intelligence.
&
%% A3
Donald Trump and his group claimed that there is no contact with Russian officials during his last year's campaign. 
&
%% A4
Russian intelligence officials made repeated contact with members of President Trump's campaign staff, according to new reports that cite anonymous U.S. officials. American agencies were concerned about the contacts but haven't seen proof of collusion between the campaign and the Russian security apparatus.
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\midrule
\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 & \multicolumn{2}{c|}{$\mathbf{D_1}$} &
\multicolumn{2}{c}{$\mathbf{D_2}$} \\
\cmidrule{1-5}
%% Sample 2
\multirow{4}{*}{$\mathbf{2}$} & 
\multicolumn{2}{C{8cm}|}{
% %% -----------------------------------------
%% D1
John McCain is out of McConnell's clutches for a week or two. 
\hlgreen{
While Sen. John McCain remains in Arizona recovering from Friday's craniotomy, surgery to remove a 5 cm blood clot from above his left eye}, business will not go on as usual in Washington. 
\hlgreen{
Majority Leader Mitch McConnell, who has to have every Republican senator voting to have a prayer of passing Trumpcare, has postponed the vote for the week or two (more likely two) that McCain's recovery will take.
}
That means there's more time for opponents to fight this thing, from the side of all of us trying to keep 22 million people from losing insurance and from the other side. 
$\mathbf{\dotso}$
% A vocal conservative opponent of the measure, Sen. Rand Paul, predicted the delay would strengthen critics' position by giving them more time to mobilize against the bill. 
% "The longer the bill is out there, the more conservative Republicans are going to discover it is not repeal," Paul (R-Ky.) said Sunday in an interview with CBS's "Face the Nation." 
% Paul is also speaking for popular vote loser Donald Trump, who he says is all for the idea of repealing everything now and replacing later. 
% Trump himself hasn't said that, but rather spent Sunday in "an angry morning tweetstorm about Hillary Clinton, the Russia controversy and other topics." 
% It seems that healthcare policy isn't at the forefront of Trump's thoughts these days. 
% Meanwhile, the so-called Republican moderates are going to be subject to intense pressure from their constituents to kill this thing, and from McConnell.
\hlgreen{With both Paul and Sen. Susan Collins (R-ME) solid "no" votes on the bill}, opponents only need one more out of the eight or so who've expressed reservations about the bill and the secretive, exclusive process McConnell
%% -----------------------------------------
} &
\multicolumn{2}{C{8cm}}{
%% -----------------------------------------
%% D2
\hlgreen{WASHINGTON - The Republican effort to repeal and replace Obamacare faces a major setback as Sen. John McCain, R-Ariz., left the nation's capital for surgery on his eye. 
Over the weekend, Senate Majority Leader Mitch McConnell, R-Ky., announced the scheduled Better Care Act vote would be delayed indefinitely because of McCain's absence.}
Subsequently, the Congressional Budget Office (CBO) also delayed its analysis of the bill. 
\hlgreen{With two Republican senators opposed to the measure, McConnell needs as least 50 "yes" votes to pass it.}
\hlgreen{Sen. Rand Paul, R-Ky., says the bill, which keeps taxes on investments and other pieces of Obamacare, doesn't go far enough. 
Moderate Sen. Susan Collins, R-Maine, is also withholding her support because it would slow the rate of growth in spending on Medicaid.}
$\mathbf{\dotso}$
% "This bill would make sweeping cuts to the Medicaid program, which has been a staple for 50 years," Collins said Sunday on ABC's "This Week with George Stephanopoulos." 
% McCain and eight others have expressed doubts about the bill and if they vote "no," it will fail. 
% With the vote now tabled, there's even more pressure on lawmakers to deliver on something many of them have promised for years: repealing and replacing Obamacare, which they warn is collapsing. 
% Some say if this bill doesn't pass, they'll have to come up with a different plan.
%% -----------------------------------------
} \\
\cmidrule{2-5}
& \multicolumn{4}{c}{\textbf{Overlap}} \\
& \multicolumn{1}{c}{\textbf{A\textsubscript{1}}} &
  \multicolumn{1}{c}{\textbf{A\textsubscript{2}}} &
  \multicolumn{1}{c}{\textbf{A\textsubscript{3}}} &
  \multicolumn{1}{c}{\textbf{AllSides}}
  \\

% \multicolumn{1}{c}{\multirow{2}{*}{$\mathbf{D_1}$}} &
% \multicolumn{1}{c}{\multirow{2}{*}{$\mathbf{D_2}$}} &
% \multicolumn{4}{c}{\textbf{Overlap}} \\
% &&\multicolumn{1}{c}{\textbf{A\textsubscript{1}}} &
%  \multicolumn{1}{c}{\textbf{A\textsubscript{2}}} &
%  \multicolumn{1}{c}{\textbf{A\textsubscript{3}}} &
%  \multicolumn{1}{c}{\textbf{AllSides}}
% \\
\cmidrule{2-5}
&
%% A1
Sen. John McCain remains in Arizona recovering from eye surgery. Senate Majority Leader Mitch  McConnell postponed the vote due to McCain's absence. Two Republican senators opposed to the bill. Possibility of bill failing.
&
%% A2
Sen. John McCain remains unavailable because of the surgery on his eye. Senate Majority Leader Mitch McConnell delayed the vote in his absence. Sen. Rand Paul and Sen. Susan Collins said "no" votes on the bill.
&
%% A3
Senate Majority Leader Mitch McConnell, R-Ky., announced the scheduled health care vote would be delayed indefinitely because of McCain's absence.
&
%% A4
Senate Majority Leader Mitch McConnell, R-Ky., announced the scheduled Better Care Act vote would be delayed indefinitely because of McCain's absence.
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% -----------------------------------------
\bottomrule
\end{tabular}
}
\caption{Some examples of \textit{TextOverlap} from 3 human annotators (\textbf{A\textsubscript{i}}) and the AllSides ``theme-description'' for a given document pair $\{D_1, D_2\}$. 
($\mathbf{\dotso}$) denotes some the sentences which for not shown for brevity.
More examples can be found in supplementary folder. 
As we notice, AllSides ``theme-description'' is only a proxy overlap summary of the input document pairs. 
Thus, having human annotators becomes critical but it a laborious and time-consuming part on humans end. Thus, lack of available dataset is a huge challenge for MNSO task. 
% ($\mathbf{\dotso}$) denotes some the sentences which for not shown for brevity.
}
\label{tab:qualitative_analysis}
\vspace{-4mm}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> SOFSAT Evaluation ARR/Tables/kendall_reward.tex <==
\begin{table*}[!htb]\footnotesize
\centering
\adjustbox{max width=\textwidth}{%
% \begin{tabular}{p{1.3cm}cccccccc}
\begin{tabular}{p{1.9cm}lccccccc}
%% ------------------------------
%% SIM 3
\toprule
\multicolumn{2}{c}{\multirow{2}{*}{\textbf{Reward/Kendall}}} &
% \multirow{2}{*}{\parbox{1.9cm}{\textbf{Sentence Embedding}}} 
\multicolumn{7}{c}{\textbf{Machine-Human Agreement in terms of Reward Function}}  \\
\cmidrule{3-9}
\multicolumn{2}{c}{} &
\multicolumn{1}{c}{$\mathbf{T=(25, 75)}$} & \multicolumn{1}{c}{$\mathbf{T=(35, 65)}$} & \multicolumn{1}{c}{$\mathbf{T=(45, 75)}$}& \multicolumn{1}{c}{$\mathbf{T=(55, 65)}$} & \multicolumn{1}{c}{$\mathbf{T=(55, 75)}$} & \multicolumn{1}{c}{$\mathbf{T=(55, 80)}$} & \multicolumn{1}{c}{$\mathbf{T=(60, 80)}$}\\ 
\midrule
% \multicolumn{9}{c}{\textbf{\textit{Sentence Embedding: P-V1}}}  \\
% \midrule

\multirow{2}{*}{\parbox{1.9cm}{\textbf{Embedding: P-v1}}} 
& \textbf{Precision} & $0.75 / 0.57$ & $0.8/0.63$ & $0.76/0.59$ & $0.8/0.63$ & $0.78/0.6$ & $0.74/0.6$ & $0.73/0.58$ \\
\cmidrule{2-9}
%----------
& \textbf{Recall} & $0.66/0.54$ & $0.76/0.64$ & $0.73/0.66$ & $0.72/0.64$ & $0.69/0.63$ & $0.65/0.64$ & $0.61/0.6$ \\
% %% ------------------------------
\midrule
% %% ------------------------------
% %% SIM 4
% \multicolumn{9}{c}{\textbf{\textit{Sentence Embedding: STSB}}}  \\
% \midrule
\multirow{2}{*}{\parbox{1.9cm}{\textbf{Embedding: STSB}}} 
& \textbf{Precision} & $0.73/0.6$ & $0.73/0.62$ & $0.73/0.6$ & $0.73/0.62$ & $0.73/0.63$ & $0.73/0.59$ & $0.73/0.58$ \\
\cmidrule{2-9}
%----------
& \textbf{Recall} & $0.63/0.55$ & $0.64/0.63$ & $0.63/0.6$ & $0.65/0.61$ & $0.65/0.61$ & $0.63/0.61$ & $0.64/0.59$ \\
%% ------------------------------
\midrule
%% ------------------------------
%% SIM 
% \multicolumn{9}{c}{\textbf{\textit{Sentence Embedding: USE}}}  \\
% \midrule
\multirow{2}{*}{\parbox{1.9cm}{\textbf{Embedding: USE}}} 
& \textbf{Precision} & $0.76/0.64$ & $0.76/0.66$ & $0.78/0.64$ & $0.78/0.64$ & $0.79/0.63$ & $0.78/0.62$ & $0.79/0.65$ \\
\cmidrule{2-9}
%----------
& \textbf{Recall} & $0.63/0.53$ & $0.66/0.6$ & $0.67/0.58$ & $0.68/0.61$ & $0.67/0.62$ & $0.64/0.62$ & $0.65/0.61$ \\
%% ------------------------------

% Kendall Results
%% ------------------------------------------------------------
\bottomrule
\end{tabular}
}
\vspace{-2mm}
\caption{
Average Precision and Recall correlation (Reward score/Kendall correlation) between label-annotators (L\textsubscript{i}) and automatically inferred labels using SEM-F1 (average of 3 label annotators). 
The raw numbers for each annotators can be found in appendix (table \ref{tab:raw_average_rewards}). 
The results are shown for different embedding models (\ref{subsec:sem_f1_evaluation}) and multiple threshold levels $T=(t_l, t_u)$. 
% For all the annotators L\textsubscript{i} ($i \in \{1, 2, 3\}$), correlation numbers are quite high ($\geq 0.50$).
Moreover, the both the Reward and Kendall values are consistent/stable across all the $5$ embedding models and threshold values.
}
\label{tab:average_rewards}
\vspace{-1mm}
\end{table*}

==> SOFSAT Evaluation ARR/Tables/notations.tex <==

% \vspace{-3mm}
\begin{table}[!htb]\footnotesize%\scriptsize
\centering
% \vspace{0mm}
% \ra{1.1}
% \resizebox{\columnwidth}{!}{%
\begin{tabularx}{\columnwidth}{lX}
\toprule
Notations & Description \\ 
\midrule
% $A \coloneqq \{ S_R \}$ & Set of reference summaries, $S_R$ (3 human and 1 AllSides) \\ 
% $GT$ & Concatenation of all the reference summaries \\ 
$S_G$ & Machines generated summary \\ 
$S_R$ & Reference summary \\ 
$T \coloneqq (t_l, t_u)$ & Tuple representing the lower and upper threshold values (between 0 and 1). \\ 
$M_E$ & Sentence embedding model \\
% $pL, rL$ & Precision and Recall labels for each sentence in $S_G$ and $S_R$ respectively \\
$pV, rV$ & Precision, Recall value for $(S_G, S_R)$ pair \\
% $I$ & Information function (either a human for manual annotation ($I_H$) or similarity metric for automatic evaluation ($I_{Sim}$)) \\ 
\bottomrule

\end{tabularx}
% }
\vspace{-2mm}
\caption{Table of notations for algorithm \ref{algo:automatic_evaluation}}
\label{tab:symbol_table}
\vspace{-5mm}
\end{table}

==> SOFSAT Evaluation ARR/Tables/reward_based_agreement.tex <==
\begin{table}[!t]\small%[!htb]
% \begin{subtable}[h]{1.0\columnwidth}
\centering
\adjustbox{max width=\columnwidth}{%
\begin{tabular}{cccccc}
\toprule
\multicolumn{6}{c}{\textbf{Human agreement in terms of Reward function}} \\
\cmidrule{2-6}
& \multicolumn{2}{c}{\textbf{Precision}} && \multicolumn{2}{c}{\textbf{Recall}} \\ \midrule
& L\textsubscript{1} & L\textsubscript{2} && L\textsubscript{1} & L\textsubscript{2} \\
\cmidrule{2-3} \cmidrule{5-6} 
%L\textsubscript{1} & --- &  &  && --- & &  \\ 
L\textsubscript{2} & $\SI{0.81 \pm 0.26}{}$ & --- && $\SI{0.85 \pm 0.11}{}$ & ---\\
L\textsubscript{3} & $\SI{0.79 \pm 0.26}{}$ & $\SI{0.7 \pm 0.31}{}$ && $\SI{0.8 \pm 0.16}{}$ & $\SI{0.77 \pm 0.17}{}$\\ 

\cmidrule{1-6}
\textbf{Average} & 
\multicolumn{2}{c}{$\mathbf{0.77}$} &&
\multicolumn{2}{c}{$\mathbf{0.81}$} \\
\bottomrule
\end{tabular}
}
\vspace{-2mm}
\caption{Average precision and recall reward scores (mean $\pm$ std) between sentence-wise annotation for different annotators. L\textsubscript{i} refers to the $i^{th}$ label-annotator.}
\label{tab:sentence-wise-annotation-agreeement}
% \vspace{-2mm}
\end{table}

==> SOFSAT Evaluation ARR/Tables/reward_function.tex <==
% Reward Table

\begin{table}[!t]\scriptsize
\centering
% \resizebox{\columnwidth}{!}{%
\begin{tabular}{c|c|ccc}
\toprule

\multicolumn{2}{c|}{\textbf{Label from Annotator B}} &  P   & PP  & A \\\cmidrule{1-5}
\multirow{3}{*}{\parbox{1.7cm}{\textbf{Label from Annotator A}}} & P                        & 1   & 0.5 & 0 \\ 
& PP                       & 0.5 & 1   & 0 \\ 
& A                        & 0   & 0   & 1 \\ 
\bottomrule
\end{tabular}
% }
% \vspace{-1mm}
\caption{Reward function used to evaluate the labels assigned by two label annotators (or labels inferred using SEM-F1 metric and human annotated labels) for a given sentence (association between annotator pairs).}
\label{tab:reward_table}
\vspace{-2mm}
\end{table}

==> SOFSAT Evaluation ARR/Tables/rouge_correlation.tex <==

% \vspace{-2mm}
\begin{table}[!t]%[!htb]
\centering
% \ra{1.1}
\begin{adjustbox}{width=\linewidth,center}
\begin{tabular}{cccccccccccc}
\toprule
\multicolumn{12}{c}{\textbf{Pearson's Correlation Coefficients}} \\ \cmidrule{1-12}
& \multicolumn{3}{c}{\textbf{R1}} &  %\phantom{abc}  
& \multicolumn{3}{c}{\textbf{R2}} &  %\phantom{abc} 
& \multicolumn{3}{c}{\textbf{RL}} \\ 
\midrule
 & I\textsubscript{1} & I\textsubscript{2} & I\textsubscript{3} &&
I\textsubscript{1} & I\textsubscript{2} & I\textsubscript{3} &&
I\textsubscript{1} & I\textsubscript{2} & I\textsubscript{3}  \\
\cmidrule{1-4} \cmidrule{5-8} \cmidrule{9-12}
%I\textsubscript{1} & ---     &   &   && ---     &   &   && --- &  &  \\ 
I\textsubscript{2} & $\mathbf{0.62}$   & ---     &   && $\mathbf{0.65}$   & ---     &   && $\mathbf{0.69}$   & ---     &   \\ 
I\textsubscript{3} & $\mathbf{0.3}$  & $\mathbf{0.38}$   & ---     && $\mathbf{0.27}$  & $\mathbf{0.37}$  & --- && $\mathbf{0.27}$  & $\mathbf{0.44}$  & ---    \\ 
I\textsubscript{4} & $\mathbf{0.17}$   & $\mathbf{0.34}$  & $\mathbf{0.34}$    && $0.14$  & $\mathbf{0.33}$   & $\mathbf{0.21}$   && $\mathbf{0.18}$   & $\mathbf{0.35}$  & $\mathbf{0.33}$  \\
\cmidrule{1-12}
\textbf{Average} & 
\multicolumn{3}{c}{\textbf{0.36}} &&
\multicolumn{3}{c}{\textbf{0.33}} &&
\multicolumn{3}{c}{\textbf{0.38}} \\

% \toprule

% %% p-values 
% \multicolumn{15}{c}{\textbf{Percentage p-values}} \\ 
% \midrule
% % \multicolumn{4}{|c|}{Rouge 1} & \multicolumn{4}{|c|}{Rouge 2} & \multicolumn{4}{|c|}{Rouge L} \\ \hline
% A\textsubscript{1} & ---     &   & & && ---  & & & && ---  & & & \\
% A\textsubscript{2} & \textbf{0.00}  & --- &  & && \textbf{0.00}  & --- & & && \textbf{0.00}  & --- & & \\ 
% A\textsubscript{3} & 1.16  & 0.00  & --- & && 0.77  & 0.00  & --- & && 0.25  & 0.00  & ---    &  \\ 
% A\textsubscript{4} & 4.14  & 0.01  & 0.00 & ---    && \textcolor{red}{10.69}  & 0.01  & 1.42 & ---    && 4.02  & 0.00  & 0.01 & --- \\ 
\bottomrule
\end{tabular}
\end{adjustbox}
% \vspace{-2mm}
\caption{Max (across 3 models) Pearson's correlation between the $F_1$ ROUGE scores corresponding to different annotators. 
Here I\textsubscript{i} refers to the $i^{th}$ annotator where $i \in \{ 1, 2, 3, 4 \}$ and ``Average'' row represents average correlation of the max values across annotators. 
Boldface values are statistically significant at p-value $<0.05$. 
For $5$ out of $6$ annotator pairs, the correlation values are quite small ($\leq 0.50$), thus, implying the poor inter-rated agreement with regards to ROUGE metric.}
\vspace{-2mm}
\label{tab:inter_annotator_agreement_rouge}
\end{table} 

==> SOFSAT Evaluation ARR/Tables/rouge_scores.tex <==
% Rouge Scores
\begin{table}[!htb]\footnotesize %scriptsize
\centering
\vspace{-2mm}
% \begin{adjustbox}{width=\linewidth,center}
\begin{tabular}{cccc}
\toprule
\textbf{Model} & \textbf{R1} & \textbf{R2} & \textbf{RL} \\
\midrule
% BART & 31.7/72.3/40.73 & 20.23/50.35/25.97 
% & 22.95/57.24/29.95 \\
% T5 & 28.1/75.97/38.50 & 17.75/55.52/24.63 & 19.93/59.48/27.73 \\
% Pegasus & 46.13/54.29/46.36 & 28.59/37.47/29.12 & 35.14/48.76/37.41 \\
BART & 40.73 & 25.97 
& 29.95 \\
T5 & 38.50 & 24.63 & 27.73 \\
Pegasus & 46.36 & 29.12 & 37.41 \\
\bottomrule
\end{tabular}
% \end{adjustbox}
\vspace{-2mm}
\caption{Average ROUGE-F1 Scores for all the test models across test dataset. For a particular sample, we take the maximum value out of the $4$ F1 scores corresponding to the 4 reference summaries. }
\vspace{-2mm}
\label{tab:rouge_score}
\vspace{-3mm}
\end{table}

==> SOFSAT Evaluation ARR/Tables/sem_f1_correlation.tex <==
% Inter-annotator agreement among SEM-F1 scores
\begin{table}[!t]\footnotesize
% \vspace{-2mm}
\centering
\begin{adjustbox}{width=\linewidth,center}
\begin{tabular}{cccccccccccc}
\toprule
\multicolumn{12}{c}{\textbf{Pearson's Correlation Coefficients}} \\ \cmidrule{1-12}
& \multicolumn{3}{c}{\textbf{P-V1}} &  %\phantom{abc}  
& \multicolumn{3}{c}{\textbf{STSB}} &  %\phantom{abc} 
& \multicolumn{3}{c}{\textbf{USE}} \\ 
\midrule
 & I\textsubscript{1} & I\textsubscript{2} & I\textsubscript{3} &&
I\textsubscript{1} & I\textsubscript{2} & I\textsubscript{3} &&
I\textsubscript{1} & I\textsubscript{2} & I\textsubscript{3}  \\
\cmidrule{1-4} \cmidrule{5-8} \cmidrule{9-12}
%I\textsubscript{1} & ---     &   &   && ---     &   &   && --- &  &  \\ 
I\textsubscript{2} & $\mathbf{0.69}$   & ---     &   && $\mathbf{0.65}$   & ---     &   && $\mathbf{0.71}$   & ---     &   \\ 
I\textsubscript{3} & $\mathbf{0.40}$  & $\mathbf{0.50}$   & ---     && $\mathbf{0.50}$  & $\mathbf{0.52}$  & --- && $\mathbf{0.51}$  & $\mathbf{0.54}$  & ---    \\ 
I\textsubscript{4} & $\mathbf{0.33}$   & $\mathbf{0.44}$  & $\mathbf{0.60}$    && $\mathbf{0.33}$  & $\mathbf{0.36}$   & $\mathbf{0.56}$   && $\mathbf{0.37}$   & $\mathbf{0.42}$  & $\mathbf{0.66}$  \\
\cmidrule{1-12}
\textbf{Average} & 
\multicolumn{3}{c}{\textbf{0.49}} &&
\multicolumn{3}{c}{\textbf{0.49}} &&
\multicolumn{3}{c}{\textbf{0.54}} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\vspace{-2mm}
\caption{Max (across 3 models) Pearson's correlation between the SEM-F1 scores corresponding to different annotators. 
Here I\textsubscript{i} refers to the $i^{th}$ annotator where $i \in \{ 1, 2, 3, 4 \}$ and ``Average'' row represents average correlation of the max values across annotators.
All values are statistically significant at p-value $<0.05$.
% For $5$ out of $6$ annotator pairs, the correlation values are quite small ($\leq 0.50$), thus, implying the poor inter-rated agreement with regards to the Rouge metric.
}
\label{tab:inter_annotator_agreement_sem-f1}
% \vspace{-2mm}
\end{table} 

==> SOFSAT Evaluation ARR/Tables/sem_f1_scores.tex <==

\begin{table}[!t]%[!htb]
% \vspace{-2mm}
\centering
\adjustbox{max width=\linewidth}{%
\begin{tabular}{cccccccccccc}
\toprule
& \multicolumn{3}{c}{\textbf{Random Annotation}} & &
\multicolumn{3}{c}{\textbf{Random Intersection}} & &
\multicolumn{3}{c}{\textbf{SEM-F1 Scores}}\\
& \multicolumn{3}{c}{\textbf{SEM-F1 Scores}} & &
\multicolumn{3}{c}{\textbf{SEM-F1 Scores}} & &
\multicolumn{3}{c}{\textbf{}}\\
\midrule
& \textbf{P-V1} &  \textbf{STSB} & \textbf{USE} & & 
\textbf{P-V1} &  \textbf{STSB} & \textbf{USE} & & 
\textbf{P-V1} &  \textbf{STSB} & \textbf{USE} \\

\cmidrule{2-4} \cmidrule{6-8} \cmidrule{10-12}
\textbf{BART} & $0.16$ & $0.21$ & $0.22$ & &
$0.21$ & $0.27$ & $0.27$ & & 
$0.65$ & $0.67$ & $0.67$ \\

\textbf{T5} & $0.17$ & $0.21$ & $0.23$ & &
$0.20$ & $0.26$ & $0.26$ & &
$0.58$ & $0.60$ & $0.60$ \\

\textbf{Pegasus} & $0.15$ & $0.20$ & $0.22$ & &
$0.19$ & $0.26$ & $0.26$ & &
$0.59$ & $0.60$ & $0.62$ \\

\cmidrule{1-12}
\textbf{Average} & $0.16$ & $0.21$ & $0.22$ & &
$0.20$ & $0.26$ & $0.26$ & &
$0.61$ & $0.62$ & $0.63$ \\
\bottomrule
\end{tabular}
}
\vspace{-2mm}
\caption{SEM-F1 Scores}
% \vspace{-1mm}
\label{tab:sem_f1_scores}
\end{table}

==> SOFSAT Evaluation ARR/Tables/sentence_wise_scoring_kendall.tex <==
%% Inter-Agreement using Kendall Correlation
\begin{table}[!t]\scriptsize
\centering
% \resizebox{\columnwidth}{!}{

\begin{tabular}{cccccc}
\toprule
\multicolumn{6}{c}{\textbf{Human agreement in terms of Kendall's Rank Correlation}} \\
\cmidrule{2-6}
& \multicolumn{2}{c}{\textbf{Precision}} && \multicolumn{2}{c}{\textbf{Recall}} \\ \midrule
& L\textsubscript{1} & L\textsubscript{2} && L\textsubscript{1} & L\textsubscript{2} \\
\cmidrule{2-3} \cmidrule{5-6} 
%L\textsubscript{1} & --- &  &  && --- & &  \\ 
L\textsubscript{2} & $0.68$ & --- && $0.75$ & ---\\
L\textsubscript{3} & $0.59$ & $0.64$ && $0.69$ & $0.71$\\ 

\cmidrule{1-6}
\textbf{Average} & 
\multicolumn{2}{c}{$\mathbf{0.64}$} &&
\multicolumn{2}{c}{$\mathbf{0.72}$} \\

\bottomrule
\end{tabular}

% \vspace{-1mm}
\caption{Average precision and recall Kendall rank correlation coefficients between sentence-wise annotation for different annotators. L\textsubscript{i} refers to the $i^{th}$ label annotator.
All values are statistically significant (p<0.05).}
\label{tab:kendall-sentence-wise-annotation-agreeement}
\vspace{-4mm}
\end{table}

==> SOFSAT Evaluation ARR/reward_correlation_table.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SEM 1 = Metric_infersent_sim_v1
\begin{table*}%[H]
%% sim_met 1 - InferSent-V1
\begin{subtable}[h]{\textwidth}
\centering
\ra{1.5}
\adjustbox{max width=\textwidth}{%
\begin{tabular}{l|r|rrr|rrr|rrr|rrr|rrr|rrr|rrr}
\hline
\multicolumn{2}{l|}{\textbf{\textit{InferSent-V1}}} & \multicolumn{ 3}{c|}{$\mathbf{T=(25, 75)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(35, 65)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(45, 75)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(55, 65)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(55, 75)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(55, 80)}$} & \multicolumn{ 3}{c}{$\mathbf{T=(60, 80)}$} \\ \hline
\hline

%% Annotator row
%% Precision
\multicolumn{2}{l|}{} & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ \\ \hline
%% Precision
\multicolumn{ 1}{l|}{\textbf{Precision}} & $A_1$ &  --- & & & --- & & & --- & & & --- & & & --- & & & --- &  &  & --- &  &  \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Reward}} & $A_2$ & 0.69 & --- & & 0.71 & --- & & 0.69 & --- &  & 0.71 & --- &  & 0.69 & --- &  & 0.67 & --- & & 0.67 & --- & \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Correlation}} & $A_3$ & 0.66 & 0.58 & --- & 0.64 & 0.6 & --- & 0.66 & 0.58 & --- & 0.64 & 0.6 & --- & 0.66 & 0.58 & --- & 0.64 & 0.56 & --- & 0.64 & 0.56 & --- \\ \hline

\multicolumn{ 1}{l|}{\textbf{Recall}} & $A_1$ & --- &  &  & --- &  & & --- & & & --- & & & --- & & & --- & & & --- & & \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Reward}} & $A_2$ & 0.82 & --- &  & 0.81 & --- &  & 0.82 & --- & & 0.81 & --- & & 0.82 & --- & & 0.79 & --- & & 0.79 & --- &  \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Correlation}} & $A_3$ & 0.65 & 0.62 & --- & 0.67 & 0.66 & --- & 0.65 & 0.62 & --- & 0.66 & 0.66 & --- & 0.64 & 0.62 & --- & 0.6 & 0.58 & --- & 0.6 & 0.58 & --- \\ \hline
\end{tabular}
}
\caption{Precision and Recall Reward Correlation using \textit{InferSent-V1} sentence embedding model}
\label{tab:sem1_reward_correlation}
\end{subtable}
\hfill
%% sim_met 2 - InferSent-V2
\begin{subtable}[h]{\textwidth}
\centering
\ra{1.5}
\adjustbox{max width=\textwidth}{%
\begin{tabular}{l|r|rrr|rrr|rrr|rrr|rrr|rrr|rrr}
\hline
\multicolumn{2}{l|}{\textit{\textbf{InferSent-V2}}} & \multicolumn{ 3}{c|}{$\mathbf{T=(25, 75)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(35, 65)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(45, 75)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(55, 65)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(55, 75)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(55, 80)}$} & \multicolumn{ 3}{c}{$\mathbf{T=(60, 80)}$} \\ \hline
\hline

%% Annotator row
%% Precision
\multicolumn{2}{l|}{} & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ \\ \hline
%% Precision
\multicolumn{ 1}{l|}{\textbf{Precision}} & $A_1$ &  --- & & & --- & & & --- & & & --- & & & --- & & & --- &  &  & --- &  &  \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Reward}} & $A_2$ & 0.56 & --- & & 0.68 & --- & & 0.51 & --- &  & 0.61 & --- &  & 0.47 & --- &  & 0.46 & --- & & 0.47 & --- & \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Correlation}} & $A_3$ & 0.42 & 0.13 & --- & 0.47 & 0.43 & --- & 0.3 & 0.04 & --- & 0.33 & 0.43 & --- & 0.28 & 0.12 & --- & 0.28 & 0.06 & --- & 0.25 & 0.03 & --- \\ \hline

\multicolumn{ 1}{l|}{\textbf{Recall}} & $A_1$ & --- &  &  & --- &  & & --- & & & --- & & & --- & & & --- & & & --- & & \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Reward}} & $A_2$ & 0.82 & --- &  & 0.81 & --- &  & 0.8 & --- & & 0.85 & --- & & 0.84 & --- & & 0.78 & --- & & 0.8 & --- &  \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Correlation}} & $A_3$ & 0.42 & 0.4 & --- & 0.54 & 0.52 & --- & 0.45 & 0.47 & --- & 0.7 & 0.69 & --- & 0.55 & 0.56 & --- & 0.47 & 0.45 & --- & 0.55 & 0.55 & --- \\ \hline
\end{tabular}
}
\caption{Precision and Recall Reward Correlation using \textit{InferSent-V2} sentence embedding model}
\label{tab:sem2_reward_correlation}
\end{subtable}
\hfill
%% sim_met 3 - Paraphrase-V1
\begin{subtable}[h]{\textwidth}
\centering
\ra{1.5}
\adjustbox{max width=\textwidth}{%
\begin{tabular}{l|r|rrr|rrr|rrr|rrr|rrr|rrr|rrr}
\hline
\multicolumn{2}{l|}{\textit{\textbf{Paraphrase-V1}}} & \multicolumn{ 3}{c|}{$\mathbf{T=(25, 75)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(35, 65)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(45, 75)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(55, 65)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(55, 75)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(55, 80)}$} & \multicolumn{ 3}{c}{$\mathbf{T=(60, 80)}$} \\ \hline
\hline

%% Annotator row
%% Precision
\multicolumn{2}{l|}{} & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ \\ \hline
%% Precision
\multicolumn{ 1}{l|}{\textbf{Precision}} & $A_1$ &  --- & & & --- & & & --- & & & --- & & & --- & & & --- &  &  & --- &  &  \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Reward}} & $A_2$ & 0.53 & --- & & 0.5 & --- & & 0.47 & --- &  & 0.51 & --- &  & 0.49 & --- &  & 0.52 & --- & & 0.55 & --- & \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Correlation}} & $A_3$ & 0.36 & 0.07 & --- & 0.31 & 0.06 & --- & 0.27 & -0.05 & --- & 0.35 & 0.04 & --- & 0.35 & -0.02 & --- & 0.39 & 0.01 & --- & 0.53 & 0.24 & --- \\ \hline

\multicolumn{ 1}{l|}{\textbf{Recall}} & $A_1$ & --- &  &  & --- &  & & --- & & & --- & & & --- & & & --- & & & --- & & \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Reward}} & $A_2$ & 0.76 & --- &  & 0.74 & --- &  & 0.66 & --- & & 0.89 & --- & & 0.87 & --- & & 0.83 & --- & & 0.86 & --- &  \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Correlation}} & $A_3$ & 0.4 & 0.43 & --- & 0.42 & 0.46 & --- & 0.55 & 0.59 & --- & 0.7 & 0.64 & --- & 0.64 & 0.6 & --- & 0.56 & 0.59 & --- & 0.67 & 0.67 & --- \\ \hline
\end{tabular}
}
\caption{Precision and Recall Reward Correlation using \textit{Paraphrase-V1} sentence embedding model}
\label{tab:sem3_reward_correlation}
\end{subtable}
\hfill
%% sim_met 4 - STSB
\begin{subtable}[h]{\textwidth}
\centering
\ra{1.5}
\adjustbox{max width=\textwidth}{%
\begin{tabular}{l|r|rrr|rrr|rrr|rrr|rrr|rrr|rrr}
\hline
\multicolumn{2}{l|}{\textit{\textbf{STSB}}} & \multicolumn{ 3}{c|}{$\mathbf{T=(25, 75)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(35, 65)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(45, 75)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(55, 65)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(55, 75)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(55, 80)}$} & \multicolumn{ 3}{c}{$\mathbf{T=(60, 80)}$} \\ \hline
\hline

%% Annotator row
%% Precision
\multicolumn{2}{l|}{} & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ \\ \hline
%% Precision
\multicolumn{ 1}{l|}{\textbf{Precision}} & $A_1$ &  --- & & & --- & & & --- & & & --- & & & --- & & & --- &  &  & --- &  &  \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Reward}} & $A_2$ & 0.49 & --- & & 0.45 & --- & & 0.49 & --- &  & 0.35 & --- &  & 0.36 & --- &  & 0.37 & --- & & 0.42 & --- & \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Correlation}} & $A_3$ & 0.35 & -0.01 & --- & 0.29 & -0.01 & --- & 0.28 & -0.05 & --- & 0.25 & 0.03 & --- & 0.33 & 0.05 & --- & 0.34 & 0.05 & --- & 0.32 & 0.08 & --- \\ \hline

\multicolumn{ 1}{l|}{\textbf{Recall}} & $A_1$ & --- &  &  & --- &  & & --- & & & --- & & & --- & & & --- & & & --- & & \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Reward}} & $A_2$ & 0.74 & --- &  & 0.67 & --- &  & 0.64 & --- & & 0.81 & --- & & 0.77 & --- & & 0.73 & --- & & 0.81 & --- &  \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Correlation}} & $A_3$ & 0.52 & 0.54 & --- & 0.35 & 0.33 & --- & 0.34 & 0.38 & --- & 0.68 & 0.6 & --- & 0.62 & 0.6 & --- & 0.55 & 0.56 & --- & 0.59 & 0.6 & --- \\ \hline
\end{tabular}
}
\caption{Precision and Recall Reward Correlation using \textit{STSB} sentence embedding model}
\label{tab:sem4_reward_correlation}
\end{subtable}
\hfill
%% sim_met 5 - USE
\begin{subtable}[h]{\textwidth}
\centering
\ra{1.5}
\adjustbox{max width=\textwidth}{%
\begin{tabular}{l|r|rrr|rrr|rrr|rrr|rrr|rrr|rrr}
\hline
\multicolumn{2}{l|}{\textit{\textbf{USE}}} & \multicolumn{ 3}{c|}{$\mathbf{T=(25, 75)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(35, 65)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(45, 75)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(55, 65)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(55, 75)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(55, 80)}$} & \multicolumn{ 3}{c}{$\mathbf{T=(60, 80)}$} \\ \hline
\hline

%% Annotator row
%% Precision
\multicolumn{2}{l|}{} & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ \\ \hline
%% Precision
\multicolumn{ 1}{l|}{\textbf{Precision}} & $A_1$ &  --- & & & --- & & & --- & & & --- & & & --- & & & --- &  &  & --- &  &  \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Reward}} & $A_2$ & 0.54 & --- & & 0.65 & --- & & 0.48 & --- &  & 0.6 & --- &  & 0.46 & --- &  & 0.42 & --- & & 0.26 & --- & \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Correlation}} & $A_3$ & 0.36 & 0.06 & --- & 0.22 & 0.1 & --- & 0.23 & -0.02 & --- & 0.23 & 0.22 & --- & 0.28 & 0.09 & --- & 0.31 & 0.02 & --- & 0.37 & 0.12 & --- \\ \hline

\multicolumn{ 1}{l|}{\textbf{Recall}} & $A_1$ & --- &  &  & --- &  & & --- & & & --- & & & --- & & & --- & & & --- & & \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Reward}} & $A_2$ & 0.73 & --- &  & 0.77 & --- &  & 0.61 & --- & & 0.61 & --- & & 0.6 & --- & & 0.63 & --- & & 0.71 & --- &  \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Correlation}} & $A_3$ & 0.37 & 0.41 & --- & 0.3 & 0.36 & --- & 0.2 & 0.29 & --- & 0.44 & 0.33 & --- & 0.34 & 0.26 & --- & 0.32 & 0.29 & --- & 0.49 & 0.5 & --- \\ \hline
\end{tabular}
}
\caption{Precision and Recall Reward Correlation using \textit{USE} sentence embedding model}
\label{tab:sem5_reward_correlation}
\end{subtable}
\hfill
\label{tab:reward_correlation_all_metrics}
\caption{Precision and recall reward correlation scores for all the 5 sentence embedding models (section \ref{subsec:sem_f1_evaluation}).\naman{Takeaway is not clear to me since there are negative values as well}}
\end{table*}

==> reward_correlation_table.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SEM 1 = Metric_infersent_sim_v1
\begin{table*}%[H]
%% sim_met 1 - InferSent-V1
\begin{subtable}[h]{\textwidth}
\centering
\ra{1.5}
\adjustbox{max width=\textwidth}{%
\begin{tabular}{l|r|rrr|rrr|rrr|rrr|rrr|rrr|rrr}
\hline
\multicolumn{2}{l|}{\textbf{\textit{InferSent-V1}}} & \multicolumn{ 3}{c|}{$\mathbf{T=(25, 75)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(35, 65)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(45, 75)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(55, 65)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(55, 75)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(55, 80)}$} & \multicolumn{ 3}{c}{$\mathbf{T=(60, 80)}$} \\ \hline
\hline

%% Annotator row
%% Precision
\multicolumn{2}{l|}{} & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ \\ \hline
%% Precision
\multicolumn{ 1}{l|}{\textbf{Precision}} & $A_1$ &  --- & & & --- & & & --- & & & --- & & & --- & & & --- &  &  & --- &  &  \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Reward}} & $A_2$ & 0.69 & --- & & 0.71 & --- & & 0.69 & --- &  & 0.71 & --- &  & 0.69 & --- &  & 0.67 & --- & & 0.67 & --- & \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Correlation}} & $A_3$ & 0.66 & 0.58 & --- & 0.64 & 0.6 & --- & 0.66 & 0.58 & --- & 0.64 & 0.6 & --- & 0.66 & 0.58 & --- & 0.64 & 0.56 & --- & 0.64 & 0.56 & --- \\ \hline

\multicolumn{ 1}{l|}{\textbf{Recall}} & $A_1$ & --- &  &  & --- &  & & --- & & & --- & & & --- & & & --- & & & --- & & \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Reward}} & $A_2$ & 0.82 & --- &  & 0.81 & --- &  & 0.82 & --- & & 0.81 & --- & & 0.82 & --- & & 0.79 & --- & & 0.79 & --- &  \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Correlation}} & $A_3$ & 0.65 & 0.62 & --- & 0.67 & 0.66 & --- & 0.65 & 0.62 & --- & 0.66 & 0.66 & --- & 0.64 & 0.62 & --- & 0.6 & 0.58 & --- & 0.6 & 0.58 & --- \\ \hline
\end{tabular}
}
\caption{Precision and Recall Reward Correlation using \textit{InferSent-V1} sentence embedding model}
\label{tab:sem1_reward_correlation}
\end{subtable}
\hfill
%% sim_met 2 - InferSent-V2
\begin{subtable}[h]{\textwidth}
\centering
\ra{1.5}
\adjustbox{max width=\textwidth}{%
\begin{tabular}{l|r|rrr|rrr|rrr|rrr|rrr|rrr|rrr}
\hline
\multicolumn{2}{l|}{\textit{\textbf{InferSent-V2}}} & \multicolumn{ 3}{c|}{$\mathbf{T=(25, 75)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(35, 65)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(45, 75)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(55, 65)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(55, 75)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(55, 80)}$} & \multicolumn{ 3}{c}{$\mathbf{T=(60, 80)}$} \\ \hline
\hline

%% Annotator row
%% Precision
\multicolumn{2}{l|}{} & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ \\ \hline
%% Precision
\multicolumn{ 1}{l|}{\textbf{Precision}} & $A_1$ &  --- & & & --- & & & --- & & & --- & & & --- & & & --- &  &  & --- &  &  \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Reward}} & $A_2$ & 0.56 & --- & & 0.68 & --- & & 0.51 & --- &  & 0.61 & --- &  & 0.47 & --- &  & 0.46 & --- & & 0.47 & --- & \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Correlation}} & $A_3$ & 0.42 & 0.13 & --- & 0.47 & 0.43 & --- & 0.3 & 0.04 & --- & 0.33 & 0.43 & --- & 0.28 & 0.12 & --- & 0.28 & 0.06 & --- & 0.25 & 0.03 & --- \\ \hline

\multicolumn{ 1}{l|}{\textbf{Recall}} & $A_1$ & --- &  &  & --- &  & & --- & & & --- & & & --- & & & --- & & & --- & & \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Reward}} & $A_2$ & 0.82 & --- &  & 0.81 & --- &  & 0.8 & --- & & 0.85 & --- & & 0.84 & --- & & 0.78 & --- & & 0.8 & --- &  \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Correlation}} & $A_3$ & 0.42 & 0.4 & --- & 0.54 & 0.52 & --- & 0.45 & 0.47 & --- & 0.7 & 0.69 & --- & 0.55 & 0.56 & --- & 0.47 & 0.45 & --- & 0.55 & 0.55 & --- \\ \hline
\end{tabular}
}
\caption{Precision and Recall Reward Correlation using \textit{InferSent-V2} sentence embedding model}
\label{tab:sem2_reward_correlation}
\end{subtable}
\hfill
%% sim_met 3 - Paraphrase-V1
\begin{subtable}[h]{\textwidth}
\centering
\ra{1.5}
\adjustbox{max width=\textwidth}{%
\begin{tabular}{l|r|rrr|rrr|rrr|rrr|rrr|rrr|rrr}
\hline
\multicolumn{2}{l|}{\textit{\textbf{Paraphrase-V1}}} & \multicolumn{ 3}{c|}{$\mathbf{T=(25, 75)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(35, 65)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(45, 75)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(55, 65)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(55, 75)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(55, 80)}$} & \multicolumn{ 3}{c}{$\mathbf{T=(60, 80)}$} \\ \hline
\hline

%% Annotator row
%% Precision
\multicolumn{2}{l|}{} & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ \\ \hline
%% Precision
\multicolumn{ 1}{l|}{\textbf{Precision}} & $A_1$ &  --- & & & --- & & & --- & & & --- & & & --- & & & --- &  &  & --- &  &  \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Reward}} & $A_2$ & 0.53 & --- & & 0.5 & --- & & 0.47 & --- &  & 0.51 & --- &  & 0.49 & --- &  & 0.52 & --- & & 0.55 & --- & \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Correlation}} & $A_3$ & 0.36 & 0.07 & --- & 0.31 & 0.06 & --- & 0.27 & -0.05 & --- & 0.35 & 0.04 & --- & 0.35 & -0.02 & --- & 0.39 & 0.01 & --- & 0.53 & 0.24 & --- \\ \hline

\multicolumn{ 1}{l|}{\textbf{Recall}} & $A_1$ & --- &  &  & --- &  & & --- & & & --- & & & --- & & & --- & & & --- & & \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Reward}} & $A_2$ & 0.76 & --- &  & 0.74 & --- &  & 0.66 & --- & & 0.89 & --- & & 0.87 & --- & & 0.83 & --- & & 0.86 & --- &  \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Correlation}} & $A_3$ & 0.4 & 0.43 & --- & 0.42 & 0.46 & --- & 0.55 & 0.59 & --- & 0.7 & 0.64 & --- & 0.64 & 0.6 & --- & 0.56 & 0.59 & --- & 0.67 & 0.67 & --- \\ \hline
\end{tabular}
}
\caption{Precision and Recall Reward Correlation using \textit{Paraphrase-V1} sentence embedding model}
\label{tab:sem3_reward_correlation}
\end{subtable}
\hfill
%% sim_met 4 - STSB
\begin{subtable}[h]{\textwidth}
\centering
\ra{1.5}
\adjustbox{max width=\textwidth}{%
\begin{tabular}{l|r|rrr|rrr|rrr|rrr|rrr|rrr|rrr}
\hline
\multicolumn{2}{l|}{\textit{\textbf{STSB}}} & \multicolumn{ 3}{c|}{$\mathbf{T=(25, 75)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(35, 65)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(45, 75)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(55, 65)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(55, 75)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(55, 80)}$} & \multicolumn{ 3}{c}{$\mathbf{T=(60, 80)}$} \\ \hline
\hline

%% Annotator row
%% Precision
\multicolumn{2}{l|}{} & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ \\ \hline
%% Precision
\multicolumn{ 1}{l|}{\textbf{Precision}} & $A_1$ &  --- & & & --- & & & --- & & & --- & & & --- & & & --- &  &  & --- &  &  \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Reward}} & $A_2$ & 0.49 & --- & & 0.45 & --- & & 0.49 & --- &  & 0.35 & --- &  & 0.36 & --- &  & 0.37 & --- & & 0.42 & --- & \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Correlation}} & $A_3$ & 0.35 & -0.01 & --- & 0.29 & -0.01 & --- & 0.28 & -0.05 & --- & 0.25 & 0.03 & --- & 0.33 & 0.05 & --- & 0.34 & 0.05 & --- & 0.32 & 0.08 & --- \\ \hline

\multicolumn{ 1}{l|}{\textbf{Recall}} & $A_1$ & --- &  &  & --- &  & & --- & & & --- & & & --- & & & --- & & & --- & & \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Reward}} & $A_2$ & 0.74 & --- &  & 0.67 & --- &  & 0.64 & --- & & 0.81 & --- & & 0.77 & --- & & 0.73 & --- & & 0.81 & --- &  \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Correlation}} & $A_3$ & 0.52 & 0.54 & --- & 0.35 & 0.33 & --- & 0.34 & 0.38 & --- & 0.68 & 0.6 & --- & 0.62 & 0.6 & --- & 0.55 & 0.56 & --- & 0.59 & 0.6 & --- \\ \hline
\end{tabular}
}
\caption{Precision and Recall Reward Correlation using \textit{STSB} sentence embedding model}
\label{tab:sem4_reward_correlation}
\end{subtable}
\hfill
%% sim_met 5 - USE
\begin{subtable}[h]{\textwidth}
\centering
\ra{1.5}
\adjustbox{max width=\textwidth}{%
\begin{tabular}{l|r|rrr|rrr|rrr|rrr|rrr|rrr|rrr}
\hline
\multicolumn{2}{l|}{\textit{\textbf{USE}}} & \multicolumn{ 3}{c|}{$\mathbf{T=(25, 75)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(35, 65)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(45, 75)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(55, 65)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(55, 75)}$} & \multicolumn{ 3}{c|}{$\mathbf{T=(55, 80)}$} & \multicolumn{ 3}{c}{$\mathbf{T=(60, 80)}$} \\ \hline
\hline

%% Annotator row
%% Precision
\multicolumn{2}{l|}{} & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ & $A_1$ & $A_2$ & $A_3$ \\ \hline
%% Precision
\multicolumn{ 1}{l|}{\textbf{Precision}} & $A_1$ &  --- & & & --- & & & --- & & & --- & & & --- & & & --- &  &  & --- &  &  \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Reward}} & $A_2$ & 0.54 & --- & & 0.65 & --- & & 0.48 & --- &  & 0.6 & --- &  & 0.46 & --- &  & 0.42 & --- & & 0.26 & --- & \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Correlation}} & $A_3$ & 0.36 & 0.06 & --- & 0.22 & 0.1 & --- & 0.23 & -0.02 & --- & 0.23 & 0.22 & --- & 0.28 & 0.09 & --- & 0.31 & 0.02 & --- & 0.37 & 0.12 & --- \\ \hline

\multicolumn{ 1}{l|}{\textbf{Recall}} & $A_1$ & --- &  &  & --- &  & & --- & & & --- & & & --- & & & --- & & & --- & & \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Reward}} & $A_2$ & 0.73 & --- &  & 0.77 & --- &  & 0.61 & --- & & 0.61 & --- & & 0.6 & --- & & 0.63 & --- & & 0.71 & --- &  \\ \cline{ 2- 23}
\multicolumn{ 1}{l|}{\textbf{Correlation}} & $A_3$ & 0.37 & 0.41 & --- & 0.3 & 0.36 & --- & 0.2 & 0.29 & --- & 0.44 & 0.33 & --- & 0.34 & 0.26 & --- & 0.32 & 0.29 & --- & 0.49 & 0.5 & --- \\ \hline
\end{tabular}
}
\caption{Precision and Recall Reward Correlation using \textit{USE} sentence embedding model}
\label{tab:sem5_reward_correlation}
\end{subtable}
\hfill
\label{tab:reward_correlation_all_metrics}
\caption{Precision and recall reward correlation scores for all the 5 sentence embedding models (section \ref{subsec:sem_f1_evaluation}).\naman{Takeaway is not clear to me since there are negative values as well}}
\end{table*}
